Overcoming High Frequency Limitations of Current-Mode Control Using a Control Conditioning Approach -- Part I: Modeling and Analysis

Current-mode control is one of the most popular controller strategies for power converters. With the advent of wide bandgap devices including GaN and SiC, higher switching frequencies have become more viable at higher power because of lower switching losses. However, the advantage of higher switching frequency for faster, higher bandwidth control is squandered because of current sensor interference. We present a framework for characterizing and analyzing this interference as uncertainties to the controller model. These uncertainties introduce additional dynamics and nonlinearity that can result in instability and poor transient performance of the current control loop. In this paper, we provide a model framework based on a new control conditioning approach that guarantees global stability and a strategy for optimizing transient performance. In Part II of this paper series, we present the analysis, design, and hardware validation of three effective solutions.

==> 4_0_general_1st_event.tex <==
\section{Control Conditioning Using Slope Compensation} \label{sec:solution}






==> 4_solution_copd.tex <==
\subsection{Comparator-Overdrive-Delay Conditioning} \label{section:opd}
In this section, we introduce a new idea using the comparator overdrive delay in real implementations of comparators to condition for interference; it is a dual-use of the comparator.  Comparator overdrive delay is a propagation delay that is dependent on the input voltage difference. In an integrated circuit, comparator overdrive delay can be made real-time programmable. 

Like other control conditioning methods, using the comparator overdrive delay can repair both the discontinuity and nonlinearity problems in static mapping along with improving the transient performance of dynamical mapping.  Comparator overdrive decreases the degree of nonlinearity in the defective static mapping shown in Fig.\,\ref{fig:comp_w_inf}.  For an ideal current sensor output ramp, using comparator overdrive delay does not create a nonlinearity, but instead introduces an offset in the static mapping, as shown in Fig.\,\ref{fig:comp_no_inf}.  This offset error does not affect the stability and transient performance of the current\nobreakdash-control loop.  Rather, it can be separated so that it is outside of the current\nobreakdash-control loop and thus becomes a disturbance for an outer voltage-control loop, which is often addressed by an integrator in the controller.
In practice, the lower bound on the interference frequency $\omega_{l}$ can be chosen as within the bandwidth of the outer loop.
% As long as the delay caused by the comparator overdrive is not longer than the switching period, the control bandwidth of voltage-control loop will not be affected.

For an ideal current sensor output ramp, comparator \mbox{overdrive} delay conditioning introduces a fixed delay in the dynamical mapping. For fixed-frequency power converters, this overdrive delay, together with other significant delays, which are caused by the blanking, subthreshold and signal propagation, should not exceed the duty cycle limits. Variable frequency power converters do not have this limitation.
%In high-frequency dc-dc converters, it is not accurate enough to just model the comparator as an ideal logic comparator.
% A new comparator model considering the overdrive propagation delay

In real voltage comparator implementations, the output of the comparator does not change instantaneously when the input difference crosses the voltage threshold, hence causing a delay.  The \emph{input overdrive} is defined as this voltage difference after the threshold is crossed, but before the output changes state.  The input overdrive can be positive or negative, \mbox{depending} on whether the signal is positive-going or negative-going.  For example, for peak current detection, input overdrive is when the current sensor voltage is above the voltage threshold set by the current command; for valley current detection, it is when the sensor voltage is below. 

The delay time depends on the input overdrive in what is known as \emph{comparator overdrive delay}, which is typically shown in datasheets.\footnote{The comparator overdrive delays that are indicated in datasheets often refer to the delays from a step changes in the input.  Other types of inputs can be inferred from the datasheet delays.}  In the rest of this section, we present comparator overdrive conditioning, without loss of generality, in the context of current-control loops that use peak current sensing, which are positive-going input signals.
\begin{figure}
    \centering
    \includegraphics[width=8 cm]{physicalmodelcomp.pdf}
    \caption{\label{fig:physicalmodel} A schematic of a simple three-stage comparator.}
\end{figure}
% To take the variable delay into consideration, we show the following variable delay comparator model: 

\begin{figure}
    \centering
    \includegraphics[width = 6cm]{comp_w_inf.pdf}
    \caption{Comparator overdrive decreases the degree of nonlinearity in the static current mapping.}
    \label{fig:comp_w_inf}
\end{figure}
\begin{figure}
    \centering
    \includegraphics{comp_no_inf.pdf}
    \caption{Comparator overdrive does not affect the nonlinearity of the static current mapping and only causes an offset error.}
    \label{fig:comp_no_inf}
\end{figure}
%\subsubsection{Modeling the Comparator Overdrive}
%To model the comparator overdrive, 
To illustrate our model for comparator overdrive, we \mbox{examine} the simple three-stage comparator shown in Fig.\;\ref{fig:physicalmodel}. It contains a differential-pair front end (Stage I), a \mbox{common}\nobreakdash-source amplifier (Stage II), and a logic inverter output (Stage III).
\begin{figure}
    \centering
    \includegraphics[width=8.5cm]{mathmodelcomp.pdf}
    \caption{\label{fig:mathmodel}
% Comparator model with overdrive propagation delay({\color{red}we do not need to have saturating integrator operator, use the green for ideal current ramp and black for the worst-case interference}).
% Figure about the current sensor output with the interference in our model class and the comparator overdrive. 
% $t_0$ is the \emph{crossing time}.
% $t_0^{'}$ is the \emph{triggering time}. 
% $t_0^{'}-t_0$ is the \emph{comparator overdrive delay}. 
% The time in Region I is denoted by $t_t$, the blanking time.
% In Region III, interference can be bounded from above by the \emph{upper envelope} and from below by the \emph{lower envelope}.
% $t_b$ and $t_d$ are the crossing time of the upper envelope and the lower envelope respectively.
% $\Delta t_b = t_0 - t_b$ is the \emph{crossing time deviation} from the upper envelope to the ideal current ramp.
% $\Delta t_d = t_d - t_0$ is the crossing time deviation from the lower envelope to the ideal current ramp.
% In Region IV, $t_b^{'}$ and $t_d^{'}$ are the triggering time of the lower envelope and upper envelope.
% $\delta t_b^{'} = t_0^{'} - t_b^{'}$ is the \emph{trigger time deviation} between the trajectories of the upper envelope and ideal current ramp. 
% $\delta t_d^{'} = t_d^{'} - t_0^{'}$ is the \emph{trigger time deviation} between the trajectories of the lower envelope and ideal current ramp. 
% The crossing time deviation of the worst-case interference is bounded between $\delta\,t_b$ and $\delta\,t_d$.
% As shown in the plot of the voltage of the comparator voltage,
% the trajectory of the capacitor voltage given the worst-case interference is bounded between the green dashed line.
% $t_b^{''}$ and $t_d^{''}$ are the triggering time given the worst-case interference.
% $\Delta\,t_b^{''} = t_0^{'} - t_1^{''}$ and $\Delta\,t_d^{''} =t_d^{''} - t_0^{'}$ are the triggering time deviation between the worst-case current sense output and ideal current ramp.
% We notice $\Delta\,t_b^{''} < \Delta\,t_b^{'}$ and $\Delta\,t_d^{''} < \Delta\,t_d^{'}$. This means for the worst-case current sense output, the triggering time deviation is smaller than the crossing time deviation.
(a) Comparator overdrive model for Region III.
(b) Comparator overdrive model for Region IV.
(c) Comparator input voltage. 
The four regions are divided by the time instants $t_a$, $t_b$ and $t_d$.
The blanking ends at $t_a$.
The upper envelope and lower envelope crosses the current command at $t_b$ and $t_d$ respectively.
(d) Comparator capacitor voltage.
The capacitor voltage trajectory of the upper envelope, ideal current ramp and lower envelope cross the threshold $V_{\text{trig}}$ at $t_b^{'}$, $t_0^{'}$, $t_d^{'}$ respectively.
The capacitor voltage trajectory given the worst-case interference is bounded between the green dashed line.
Hence the comparator output can not trigger earlier than $t_b^{'}$ or later than $t_d^{'}$.
{\color{red} need update $C_{\text{eff}}$ in 
the figure above}}
\end{figure}

We denote the equivalent capacitance at the output of Stage~I by $C_{\text{eff}}$. The comparator output toggles only if the voltage difference $V_{+} - V_{-}$ lasts long enough so that $C_{\text{eff}}$ is charged or discharged to cross the voltage threshold of Stage~II.
The current at the output of Stage~I is $i_{-} - i_{+}$, which can also be expressed as $g(V_{-} - V_{+})$, where $g$ is a nonlinear transconductance \cite{razavi2002design}. 
% This current charges the parallel $C_{\text{eff}}$ and $R_{\text{out}}$, which is the equivalent resistor at the output the Stage I.
Because of $R_{\text{eff}}$, which is the effective resistance at the output of Stage~I, the charging current for $C_{\text{eff}}$ is always smaller than $i_{-} - i_{+}$.
$R_{\text{eff}}$ effectively decreases the transconductance.  For the analysis, we choose a constant $G$, which is the largest small-signal transconductance in the range of $g$.  Choosing the largest transconductance results in the lowest comparator overdrive delay and hence a conservative design for stability.
% Because the tail current $i_T$ is constant, this requires including $i_T$ as the saturation capacitor current in the control conditioning model.
Because $g$ is determined by $i_T$, overdrive delay can be programmed by changing this tail current $i_T$, for example in an integrated circuit design.

% The current which charges the effective capacitor is $g(V_{+} - V_{-})$, where the $g$ is the nonlinear transconductance.
% The tail current, denoted by $i_T$, determines the speed of charging or discharging $C_{\text{eff}}$. The overdrive delay can be accurately controlled by programming the tail current $i_T$ in the integrated circuit.

%\begin{figure}
% \begin{minipage}{0.32\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{Figure/section3/OPD/OPD1.png}
%     \caption{ \label{fig:OPD1} Comparator Response time various input overdrives.}
% \end{minipage}
% ~
% \begin{minipage}{0.32\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{Figure/section3/OPD/OPD2.png}
%   \caption{  \label{fig:OPD2} Comparator Response time various input overdrives(2).}
% \end{minipage}
% ~
% \begin{minipage}{0.32\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{Figure/section3/OPD/physicalmodelcomp.pdf}
%     \caption{\label{fig:physicalmodel} Simplified physical model of a comparator.}
% \end{minipage}
%\end{figure}

% We show a mathematical model in Fig.\;\ref{fig:mathmodel} which models the physical mechanisms in Fig.\;\ref{fig:physicalmodel}.

% because the voltage %range of comparator overdrive delay is usually below 50\,mV. Within this range, the 
% transconductance can be % considered as linear. 
% The transconductance is easily programmable by tuning the tail current in either an online or offline way.
% The current sensor output and current command are put in a substractor.
% { \color{blue}
% (written by XC, to be deleted and substituted by Prof's comments)
% We define a model class for the interference which contain three regions.
% This is the only model class which we can manage and derive the global stability criterion.
% In Region A, the waveform has a severe switching transient which might saturate to the negative rail or exceed the current command threshold. We use the time blanking to avoid the
% severe switching transient. The blanking time $t_t$ corresponds the minimum on
% time for a peak current-mode controller. The blanking time is
% designed to be long enough so positive excursions do not leave
% a state on the integrator.
% In Region B, the waveform is below current command threshold and did not saturate to the negative rail. Region C is the comparator overdrive Region.

% The current sensor output with the interference satisfying our model class and the comparator overdrive
% are shown in Fig.\,\ref{fig:mathmodel}.}
% {\color{blue}
% A representative current sensor output is shown in Fig.\,\ref{fig:mathmodel}\,(b).  The interference satisfies our model class.  This model class allows us to model the comparator only for its overdrive Region, which is shown in Fig.\,\ref{fig:mathmodel}\,(a). As before, we analyze the interference as a deviation from the ramp output of an ideal current sensor. 
% }

We formulate a model class based on practical current sensor waveforms from power electronics, for example in Fig.\,\ref{fig:noisecurrent}.  This class elicits a model that is straightforward in guaranteeing global stability.

This model class is characterized by four regions, which can be observed in Fig.\,\ref{fig:mathmodel}(c).  
Region I is the ``blanking'' region, where large and very fast but quickly decaying switching transients dominate the current sensor output.  
It is worth noting that in the many instances that this region is blanked, the blanking occurs after output of the comparator to defer the peak current event detection. 
Region II is the ``subthreshold'' region where the worst-case current sensor waveform is below the current command.
Region III is the ``threshold'' region where the current sensor waveforms are neither unambiguously below nor above the current-command threshold; in this region, the waveform can cross the threshold multiple times.
Region IV is the ``overdrive'' region where the current sensor waveform is always above the current command.
The qualifying restriction on Region II, III, and IV for this model class is that waveform is never below the minimum current command.  

In Regions I and II, we consider the comparator capacitor to remain in reset or equivalently, negatively saturated. In Regions III and IV, the capacitor integrates the current that is representative of the difference between the current command and the current sensor output; the mathematical formalization requires two different types of integrators to describe each region, as shown in Fig.\,\ref{fig:mathmodel}(a) and (b).  The integrator resets every switching cycle for the usual case that the overdrive delay of the comparator is smaller than the minimum off time.
% {\color{red} (Ask professor of this sentence is needed or not) need an explanation somewhere of Fig. 37d.}

The ideal current sensor output (without interference) is a ramp, which crosses the current command threshold at $t_0$.  After $t_0$, $C_{\text{eff}}$
%the capacitor on the comparator 
begins integrating; for the ideal current ramp, the capacitor voltage is a quadratic.  When the capacitor voltage crosses the trigger voltage $V_{\text{trig}}$ at $t_0$, which results from a combination of the gains and MOSFET thresholds (for example in Fig.\,\ref{fig:physicalmodel}) for $\text{Q}_3$, the comparator output changes state at $t_0^{'}$.
The overdrive delay is from 
$t_0$ to $t_0^{'}$.
% the instant that the comparator input crosses the current command to the instant when the comparator output triggers.

The current sensor output with interference in our model class can be bounded from above by an \emph{upper envelope} and from below by a \emph{lower envelope} in Regions II and III.
The upper envelope crosses the current command earlier than the ideal current ramp by $\Delta t_b = t_0 - t_b$.
The lower envelope crosses the current command later than the ideal current ramp by $\Delta t_d = t_d - t_0$.
The upper and lower envelope  
have the same comparator overdrive delay as the ideal current ramp because these envelopes have the same slope as the ideal current ramp given the bounded amplitude assumption,
\begin{equation}
    t_0^{'} - t_0 \, = \, t_b^{'} - t_b \, = \, t_d^{'} - t_d.
\end{equation}
Although the overdrive delays are identical, the upper envelope triggers earlier than that of the ideal current ramp by $\Delta t_b^{'} = t_0^{'} - t_b^{'}$ and the lower envelope triggers later by $\Delta t_d^{'} = t_d^{'} - t_0^{'}$.

The worst-case interference waveform that can be contained by the upper and lower envelopes is a trapezoidal signal \cite{Zhang2015a}.  The lower bound $\omega_l$ of the interference frequency is the fundamental of the trapezoidal signal.  The largest slew rate of the trapezoidal signal is the upper bound of the Lipschitz constant $\Lambda_{ub}$.

Comparator overdrive conditioning decreases the trigger time deviation from the ideal ramp for waveforms within the envelope bounds. In Region III, the time deviation of the crossing event of the worst\nobreakdash-case interference from that of the ideal current ramp can range from $\Delta t^{'}_b$ earlier to $\Delta t^{'}_d$ later. In Region IV, the capacitor voltage trajectory given the worst-case interference input is strictly bounded between quadratic trajectories of the upper and lower envelope inputs.  This is a strict bound because the integral of the worst-case trapezoid is bounded from above by $\pi A_{ub} / \omega_l$; hence, the comparator output cannot trigger earlier than $\Delta t_b^{'}$ nor later than $\Delta t_d^{'}$. The tradeoff to this control conditioning method is that longer overdrive delay becomes commensurate with smaller trigger time deviation.  This overdrive delay manifests as a limitation to an outer control loop, which might for example, control output voltage.
% \red{(ask prof if this sentence is needed or not) overdrive delay -- defined by crossing to trigger time?  in terms of model}

% we formulate a model class based on practical current sensor waveforms from
% power electronics (e.g. Fig. \ref{fig:noisecurrent}).
% As shown in Fig.\,\ref{fig:mathmodel}, there is a severe switching transient at the current sensor output nearby $t = 0$.
% The current sensor output may saturate to the negative rail of comparator.
% It may also exceed the current command.
% We use the time blanking to avoid the severe switching transient.
% We denote the blanking time, $t_t$, as 
% the time after the current sensor output no longer hits the negative rail. This blanking time corresponds the minimum on time for a peak current-mode controller.
% The blanking time is designed to be long enough so positive excursions do not leave a state on the integrator.

% We denote the idealcrossing time, when the pure ramp signal crosses the current command, by $t_0$.
% Because of the interference, the actual crossing time deviates from $t_d$.

% We consider the interference which satisfies the Definition \ref{def:inteference}.
% The interference does not have a dc component.
% We further assume there is a low frequency limit of the interference $\omega_l$.
% we can draw the 
% \emph{earliest envelope line} and \emph{latest envelope line} of the current sensor output.
% Any interference is bounded between these two lines.
% The worst-case interference is a trapezoid waveform whose period is $\omega_l$ and largest slew rate is determined by the Lipschitz constant bound.
% We denote the \emph{crossing time deviation} from the earliest envelope line to the ideal ramp by $t_1$.
% The \emph{crossing time deviation} from the latest envelope line to the ideal ramp is denoted by $t_2$.
% The earliest envelope line results in the shortest  crossing time $t_0 - t_1$.
% The latest envelope line results in the longest crossing time $t_0 + t_2$.

% Before the crossing time, the current sensor output is smaller than the current command.
% The comparator capacitor is discharged and clamped to the negative rail.
% After the crossing time, the comparator capacitor starts to be charged.
% The ideal voltage trajectory is a quadratic function.
% Once the capacitor voltage is higher than the threshold voltage $V_{\text{th}}$, the output of the comparator triggers. We denote the \emph{triggering time} by $t^{'}_0$. 
% The difference between the triggering time and crossing time $t^{'}_0 - t_0$ is the ideal comparator overdrive delay.
% The quadratic capacitor voltage trajectories of the earliest triggering line and latest triggering line are shown as red in the plot of the voltage of the comparator capacitor.
% The overdrive delay of the earliest and latest envelope line is the same of the ideal comparator overdrive delay because all three lines have same slope. 
% Therefore, the triggering time of the earliest envelope line is $t_0 - t_1$ and that of the latest envelope line is $t_0 + t_1$.
% The voltage trajectory of the worst-case current sensor output is bounded by the dashed line.
% The dashed line is strictly between the voltage trajectories from the earliest envelope line and latest envelope line because the integral of the worst-case interference is bounded by $\omega_l$ and $A_{ub}$.

% We denote the \emph{triggering time deviation} between the voltage trajectory of the earliest envelope line and ideal ramp by $t^{'}_1$.
% The \emph{triggering time deviation} between the voltage trajectory of the latest envelope line and ideal ramp by $t^{'}_2$.
% We observe that $t^{'}_1 < t_1$ and $t^{'}_2 < t_2$ because the voltage trajectory of the worst-case current sensor output is strictly between those of the earliest envelope line and latest envelope line.
% In all, the comparator overdrive condition the current sensor output by decreasing the triggering time deviation from the ideal current ramp.
% The price which this method pays is the overdrive delay from the crossing time to triggering time. The longer the overdrive delay is, the smaller triggering time deviation is.



% The mathematical model Fig.\;\ref{fig:mathmodel} does not take the physical mechanism that the voltage of capacitor can be clamped by the positive or negative voltage rails of the comparator into consideration.
% The reason for saturating is because the voltage of capacitor is always clamped by the positive and negative voltage rails.
% The complete model can be found in the proofs in Appendix.
% However, it is difficult to guarantee global stability from this general model. Instead, we formulate a model class based on practical current sensor waveforms from power electronics (e.g.\,Fig.\,\ref{fig:noisecurrent}).
% {\color{red} picture remaining to be added}
% We also assume $C_{\text{eff}} V_{\text{th}} = 1$ if not specifically mentioned.
% \begin{figure}
%     \centering
%     \includegraphics[width=8 cm]{Figure/section3/opd/simumodelcomp}
%   \caption{\label{fig:odpopcomp} Comparison of the mathematical model and actual data on the overdrive-propagation delay of comparator LT1711.}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=8cm]{Figure/section3/opd/functionTOPD.pdf}
%   \caption{  \label{fig:functionT} The graphs of the function $\mathcal{T}$ of comparator OPD with different error gain. The dash-dotted blue line represents the function $\mathcal{T}$ with the OPD. The solid red line represents the function $\mathcal{T}$ with the  and the green dots represent the jump discontinuity points.}
% \end{figure}
\begin{figure*}[ht]
\centering
\subfigure[Comparison of the model and experimental data on the overdrive delay of comparator LT1711. $\Delta v$ represents the input overdrive and $t_d$ represents the delay. The fitted trigger voltage --- time constant product $V_{\text{trig}}\tau = 6.102\,$ps$\cdot$V, and $T_d = 4.198\,$ns.]
{\includegraphics[width = 0.3\textwidth ]{simumodelcomp_lt1711.pdf}
\label{fig:simumodelcomp_lt1711}
}
\subfigure[Comparison of the model and experimental data on the overdrive delay of comparator AD8469. $\Delta v$ represents the input overdrive and $t_d$ represents the delay. The fitted trigger voltage --- time constant product $V_{\text{trig}}\tau = 113.3\,$ns$\cdot$mV, and $T_d = 24.75\,$ns.]
{\includegraphics[width = 0.3\textwidth ]{simumodelcomp_ad8469.pdf}
\label{fig:simumodelcomp_ad8469}
}
\subfigure[Static mapping with different comparator overdrive delay. {\color{blue}-\,-\,-} is for the comparator with zero overdrive delay.  {\color{green}---} is for the comparator with medium overdrive delay. The jump discontinuity points are represented by {\color{red}$\cdots$}. 
  {\color{orange}-\,$\cdot$\,-} is for the comparator with long overdrive delay.]{ \includegraphics[width = 0.3\textwidth]{functionTOPD.pdf} \label{fig:functionTwOPD}
}
\caption{Comparison of the model and experimental data on the overdrive delay.}
\end{figure*}
% \begin{figure}
%   \centering
%   \includegraphics[width=8 cm]{Figure/section3/opd/simumodelcomp.pdf}
%   \caption{\label{fig:odpopcomp} Comparison of the model and experimental data on the overdrive delay of comparator LT1711 \cite{Dual2001}. $\Delta v$ represents the input overdrive and $t_d$ represents the delay. The fitted trigger voltage --- time constant product $V_{\text{trig}}\tau = 6\,$ps$\cdot$V, and $T_d = 4.18\,$ns.
% %   Note that this not the only parameter set which can fit the experimental data.
%   \newline}
% \end{figure}
% \begin{figure}
%   \centering
%   \includegraphics[width=8cm]{Figure/section3/opd/functionTOPD.pdf}
%   \caption{\label{fig:functionTwOPD} Static mapping with different comparator overdrive delay. {\color{blue}-\,-\,-} is for the comparator with zero overdrive delay.  {\color{green}---} is for the comparator with medium overdrive delay.
%   The jump discontinuity points are represented by {\color{red}$\cdots$}. 
%   {\color{orange}-\,$\cdot$\,-} is for the comparator with long overdrive delay.}
% \end{figure}

%\subsubsection{Modeling the current-controller with the %Comparator Overdrive}


%Region B/C boundary is worst-case delay.  Apply lower envelope to saturating integrator.

Delay and nonlinearity are the pertinent effects that determine stability and transient performance. Region I (blanking), Region II (subthreshold), and Region III (threshold) are modeled as pure delays in Fig.\;\ref{fig:mathmodel}(c). $T_d$ is a constant that encapsulates the circuit delays that are independent of the comparator input.  This model for comparator overdrive delay agrees well with the real-world data \cite{Dual2001} shown in Fig.\;\ref{fig:simumodelcomp_lt1711} and Fig.\;\ref{fig:simumodelcomp_ad8469}.

The model for Region III (threshold) is shown in Fig.\;\ref{fig:mathmodel}(a).  The salient feature of this model is the saturating integrator,  
whose state and hence output is bounded both from above and below, but behaves like a linear integrator between these bounds.  An implementation of a comparator with this behavior is illustrated in Fig.\,\ref{fig:physicalmodel}, where $V_c$ is always above ground.  It is worth noting that the comparator circuit actually possesses this behavior in all four of the the model regions.  Stability guarantees can be proven by partitioning the comparator behavior into these regions and restricting the saturating integrator behavior to Region III.

This saturating integrator behavior is mathematically important in that the saturating integrator is a sublinear function, which enables the proof of continuity in the static mapping in Appendix\,\ref{proof:gmaxcontinuity}.
The definitions of the saturating integrator can be found in Definition \ref{def:sat_int} in Appendix\,\ref{proof:gmaxcontinuity}.
The behavior in Region III be represented by
    \begin{align} \label{eqn:IT_reg_3} V(t) =  \frac{1}{C_{\text{eff}}}\sint_{t_b}^{t_d} G\left(i_v[n] + m_1 t + w(t) - i_c [n] \right) dt.
\end{align}
We define $t_{fi}$ as the last instant in Region III when the output of the integrator $V(t)$ is zero.\footnote{We provide a short proof for this statement: the saturating integrator always has positive or zero state at any threshold crossing instants.
We start from the last instant and backwards check the integrator states at each threshold crossing instants.
We stop at the instant at which the integrator state is zero.
This algorithm is guaranteed to stop because the integrator state must be zero at the first threshold crossing instant.
Therefore, the stop instant is the $t_{fi}$ we want.}
\begin{align} \label{eqn:final_i_eqn_num_trick}
    t_{fi} \triangleq \left\{t^\prime ~ \rvert ~~ V(t^\prime) = 0 \,\text{and}\, V(t) > 0 ~~ \forall\,t > t^\prime\right\}.
\end{align}
% because ideal current ramp is monotonically increasing and the interference is bounded 
% For any instant when the integrator is zero, a negative error will keep the state still stay at zero and a positive error will immediately push the state to positive. Therefore, a threshold crossing.
% Because the current sensor output 

After $t_{fi}$, the behavior in Region III is a linear integrator with a voltage output $V_0$ at the end of Region III
\begin{align} 
    \label{eqn:v_0_rep} 
    % \frac{1}{C_{\text{eff}}} \sint_{t_{fi}}^{t_{d}} G\left(i_v[n] + m_1 t + w(t) - i_c [n] \right) dt \nonumber \\
      V_0 = \frac{1}{C_{\text{eff}}} \int_{t_{fi}}^{t_{d}} G\left(i_v[n] + m_1 t + w(t) - i_c [n] \right)\,dt.
\end{align}

The model for Region IV (overdrive), which represents a strictly positive integrator output is modeled in Fig.\;\ref{fig:mathmodel}(b).
The initial output $V_0$ of the integrator embeds the saturating integrator behavior in Region III.
$V_0$ is bounded from above by $\frac{1}{2}m_1(t_b - t_d)^2$, which is induced by the upper envelope of the current sensor output.
$V_0$ is bounded from below by the lower bound of the saturating integrator.

The comparator overdrive in Region IV can be represented by
    \begin{align} \label{eqn:IT_new} V_{0} + \frac{1}{C_{\text{eff}}}\int_{t_d}^{t_{\text{on}}[n]} G\left(i_v[n] + m_1 t + w(t) - i_c [n] \right) dt = V_{\text{trig}}.
\end{align}
% \begin{align}
%     \sint
% \end{align}
% The algorithm to find out the $G_{\text{max}}$, the maximum gain which make the equilibrium existence condition hold can be found in appendix.
In (\ref{eqn:IT_new}),
$i_v[n] + m_1 t + w(t) - i_c [n]$ represents the error between the current sensor output and the current command.
% $\sint$ is a \emph{saturating integral operator} defined in Appendix \ref{proof:gmax4feasibility}.

% We assume that the maximum voltage difference between the comparator input $\delta v_{\text{comp}}$ is in 
% We denote the range of $g$  by $[G_{\text{min}},G]$.
% From our previous discussion of the Region III conditions, specifically,  $t_{fi}$ is the minimum solution of the equation $ m_1 t + f(t)  = i_c [n] - i_v[n]$ which satisfies
% We define the \emph{crossing time} $t_{fi}$ as the \emph{minimum solution} of the equation
% $ \label{eqn:DTC}
%  m_1 x + f(x)  = i_c [n] - i_v[n]$
% which satisfies
% \begin{align} \label{eqn:IT_nosat}
%     \frac{1}{C_{\text{eff}}} \int_{t_{fi}}^{t_{\text{on}}} g\left(i_v[n] + m_1 t + w(t) - i_c [n] \right) dt > 0, \quad \forall \; t_{\text{on}}>t_{fi}.  
% \end{align}
% By introducing $t_{fi}$, we convert the model in (\ref{eqn:IT}) which uses nonlinear saturating integral operator into the model in (\ref{eqn:IT_nosat}) which only uses linear integral operator.
By substituting (\ref{eqn:v_0_rep}) into (\ref{eqn:IT_new}), the comparator overdrive can be represented as
\begin{align} \label{eqn:IT} \frac{1}{C_{\text{eff}}}\int_{t_{fi}}^{t_{\text{on}}[n]} G\left(i_v[n] + m_1 t + w(t) - i_c [n] \right) dt = V_{\text{trig}}.
\end{align}
Together with the dynamics of the constant off-time current-control loop, the system using the comparator overdrive can be represented as
% Considering the actual peak current $i_p[n] = i_v[n] + t_{\text{on}}[n]$ and the peak current deviation $i_e[n] \triangleq i_c[n] - i_v[n]$ into (\ref{eqn:IT_nosat}), the current-control loop using comparator overdrive can be represented as
% By substituting $i_p[n] = i_v[n] + m_1t_{\text{on}}[n]$ and $i_e[n] \triangleq i_c[n] - i_v[n]$ into (\ref{eqn:IT_nosat}), the current-control loop can be represented as
\begin{subequations}
\label{eqn:opd_sys}
    \begin{align} 
    \label{eqn:ITlinear} \int_{t_{fi}}^{t_{\text{on}}[n]}
    & \left(i_v[n] + m_1 t + w(t) - i_c [n] \right) dt =  V_{\text{trig}}\tau, \\
    \label{eqn:forwardpath}
    & i_p[n] = i_p[n-1] - m_2T_{\text{off}} +m_1t_{\text{on}}[n],
    \end{align}
\end{subequations}
where the comparator time constant $\tau = C_{\text{eff}}/G$ is the {\em design variable} for comparator-overdrive-delay conditioning. Equation (\ref{eqn:ITlinear}) describes the feedback path and (\ref{eqn:forwardpath}) describes the forward path. 

Proposition\,\ref{th:equexcond} in Section\,\ref{sec:fet_latching} states that if the current sensor output is not monotonic, then the static current mapping is discontinuous.
A discontinuous static mapping can make the current-control loop unstable.
We use $\tau$  as the metric for the comparator overdrive delay. \mbox{Theorem}\,\ref{theorem:gmaxcontinuity} below states that an appropriately designed comparator overdrive delay can make the static mapping continuous.
Figure\,\ref{fig:functionTwOPD} demonstrates Theorem\,\ref{theorem:gmaxcontinuity} by plotting three static mappings with different comparator overdrive delays. 
We observe that given small $\tau$, the static mapping is discontinuous.
As we increase $\tau$, the degree of discontinuity of the static mapping decreases. The static mapping becomes continuous if $\tau$ is large enough. Mathematically, the degree of discontinuity can be defined as the Lebesgue measure on the set of unreachable points.

% From Proposition\, \ref{th:equexcond}, 
% if the current sensor output is not monotonic, the static current mapping is not continuous anymore. 
% The current-control loop may be unstable because of this discontinuity.
% The comparator overdrive delay decreases the degree of discontinuity of the static mapping so that it is continuous.
% We leverage the transconductance $G$ to adjust the overdrive delay. 
% Figure\;\ref{fig:functionTwOPD} illustrates the static current mapping $\mathcal{T}$ given the comparator with different transconductance and overdrive delay.
% % The Lebesgue measure of $U\!E$ exists and we denote it by $\lambda(U\!E)$.
% We note that as $G$ increases, the degree of the discontinuity of the static mapping decreases. 
% Therefore, we can expect that there exists a maximum error gain $G_{\text{max}}$ to guarantee the continuity condition and stability condition.

\begin{theorem} \label{theorem:gmaxcontinuity}
Given a constant off-time current-control loop with comparator overdrive delay, if the input is a ramp with slope $m_1$ and interference function $w(t)$, the condition to guarantee the continuous static current mapping is
\begin{align}
  V_{\text{trig}}\tau \ge m_1 K_3\!\left(\frac{|W(\omega)|}{m_1}\right).
\end{align}
\end{theorem}
The definition of the $K_3(\cdot)$ function as well as the proof of Theorem \ref{theorem:gmaxcontinuity} can be found in Appendix \ref{proof:gmaxcontinuity}.

Having satisfied the condition of continuous static mapping, we next show that the comparator overdrive delay allows the dynamical mapping to be stabilized even if the original interference violates the stability bound in Theorem\,\ref{theorem:gloasystab}.
Comparator overdrive conditioning attenuates the effect of interference by averaging, hence its performance improves with increasing interference frequency.  The averaging time interval is determined by $\tau$; smaller $\tau$ results in longer averaging time and hence a better interference attenuation.  Smaller $\tau$ contributes to a bigger delay, which means that interference attenuation trades off with transient performance. Theorem\,\ref{theorem:gmax4stability} describes the stability constraint on the design of $\tau$;
Theorem\,\ref{theorem:gmax4overdrivedelay} describes the constraint from the hardware limits on minimum on time.

Theorem\,\ref{theorem:gmax4stability} shows there exists a minimum comparator time constant, above which the current-control loop is guaranteed to be globally asymptotically stable.
The stability of the dynamical mapping depends on the upper bound of the interference amplitude $A_{ub}$ and the lower bound of the interference frequency $\omega_l$.  Only a short overdrive delay is needed to stabilize the current-control for small $A_{ub}$ and large $\omega_{l}$.  This is consistent with the behavior we described in Fig.\,\ref{fig:mathmodel}. 

% Given a continuous static mapping, the stability of the dynamical mapping is determined by the upper bound of the Lipschitz constant $L_{ub}$ of the interference.
% For the interference whose Lipschitz constant is outside of this bound, we show that an appropriately designed comparator overdrive delay can still guarantee the globally asymptotic stability of the current-control loop. 
% The stability condition depends on the upper bound of the amplitude of the interference $A_{ub}$ and lower bound of the frequency spectrum of the interference $\omega_l$. 
% The smaller $A_{ub}$ is, smaller $\omega_l$ is or larger $G_{\text{max}}$ is, the better stability margin the current-control loop has.
% This matches the qualitative analysis in Fig.\,\ref{fig:mathmodel}.
\begin{theorem} \label{theorem:gmax4stability}
Given a constant off-time current-control loop with comparator overdrive delay, if the input is a ramp with slope $m_1$ and interference function $w(t)$,
% maximum $T^{\text{max}}_{\text{on}}$ in the transient, 
the condition to guarantee a globally asymptotically stable dynamical mapping is
\begin{align}\label{eqn:vtrigtau_constraint}
  V_{\text{trig}} \tau \ge \frac{4A_{ub}^2}{m_1} + B,
\end{align}
where
\begin{align} 
  \tau = \frac{C_{\text{eff}}}{G}, \quad B = \int_{-\infty}^{+\infty} \Bigg| \frac{W(\omega)}{\omega}  \Bigg| \,d\omega \nonumber.
\end{align}
\end{theorem}
% The constraint (\ref{eqn:vtrigtau_constraint}) is derived from Theorem \ref{theorem:gloasystab}.
The proof of this Theorem is based on the observation that (\ref{eqn:ITlinear}) is an implicit nonlinear function from $t_{\text{on}}[n]$ to the deviation of peak current $i_c[n] - i_p[n]$. 
Therefore, the current\nobreakdash-control loop can be represented as a Lure system.
Equation (\ref{eqn:forwardpath}) describes the linear forward path and $G(z)$ can be found in (\ref{eqn:gzofcotcm}).
(\ref{eqn:ITlinear}) describes the nonlinear feedback path and $\psi(\tilde{t}_{\text{{on}}})$ is sector\nobreakdash-bounded by $[-2A_{ub}/t_{od}^{\text{min}},+\infty)$
\begin{align}
\label{eqn:sc_bd_psi_opd}
  \left( \psi(\tilde{t}_{\text{{on}}}) + \frac{A_{ub}}{t_{od}^{\text{min}}}\tilde{t}_{\text{{on}}} 
  \right) \tilde{t}_{\text{{on}}} > 0,
\end{align}
where $t_{od}^{\text{min}}$ is the minimum comparator overdrive delay, which is derived in Appendix\,\ref{proof:feedbackgain}.  The proof for stability is derived in Appendix\,\ref{proof:gmax4stability}  using Theorem\,\ref{theorem:gloasystab}.
Equation (\ref{eqn:vtrigtau_constraint}) shows that a current-control loop with large interference amplitude can be stabilized by a comparator with a large time constant $\tau$.

However, having a time constant $\tau$ that is too large results in an overdrive delay that may be too long. Long overdrive delay increases the minimum on time $T_{\text{on}}^{\text{min}}$ of the current-control loop, hence slowing down transient response. Theorem~\ref{theorem:gmax4overdrivedelay} shows a rigorous upper bound on the overdrive delay.
% design of $\tau$ given the constraint on $T_{\text{on}}^{\text{min}}$.
\begin{theorem}
\label{theorem:gmax4overdrivedelay}
Given a constant off-time current-control loop with comparator overdrive delay, if the input is a ramp with slope $m_1$ and interference function $w(t)$,
% the on time is bounded from below by $T_{\text{on}}^{\text{min}}$, 
%then a upper bound for $\tau$ is
the maximum comparator overdrive delay $t_{od}^{\text{max}}$ is
% {\color{blue} rewrite equation with $\tau$}
% \begin{align}\label{eqn:tau_constraint}
%     \frac{A_{ub}}{m_1} + \sqrt{\left(\frac{A_{ub}}{m_1}\right)^2+\frac{2}{m_1}\left(V_{\text{th}}\tau + B \right)} \le T_{\text{on}}^{\text{min}},
% \end{align}
\begin{align}\label{eqn:tau_constraint}
    t_{od}^{\text{max}} = \frac{A_{ub}}{m_1} + \sqrt{\left(\frac{A_{ub}}{m_1}\right)^2+\frac{2}{m_1}\left(V_{\text{th}}\tau + B \right)},
\end{align}
where
\begin{align}
  \tau = \frac{C_{\text{eff}}}{G}, \quad B = \int_{-\infty}^{+\infty} \Bigg| \frac{W(\omega)}{\omega}  \Bigg| \,d\omega \nonumber.
\end{align}
\end{theorem}
The maximum comparator overdrive delay $t_{od}^{\text{max}}$  depends on the interference, hardware parameters, and design variable $\tau$.
The proof of this Theorem can be found in Appendix\,\ref{proof:gmax4stability}.

The large-signal transient performance of the power converter is determined by the inductor current slew rate, which in turn is determined by the minimum on time $T_{\text{on}}^{\text{min}}$. 
$T_{\text{on}}^{\text{min}}$ is a \emph{design objective} for comparator-overdrive-delay conditioning.
We design the comparator so that $T_{\text{on}}^{\text{min}}$ is as small as possible while maintaining stability.
Therefore, a judicious choice is to design the longest overdrive delay to equal the minimum on~time
% As long as the longest overdrive propagation delay does not exceed $T_{\text{on}}^{\text{min}}$, the current command can be adjusted so that the current-control loop can stably operate at $T_{\text{on}}^{\text{min}}$. 
%The left hand side of (\ref{eqn:todmax_constraint}) is proven to be an upper bound of the overdrive delay. The detailed proof can be found in Appendix\,\ref{proof:gmax4stability}.
\begin{align}\label{eqn:todmax_tonmin}
    T_{\text{on}}^{\text{min}} = t_{od}^{\text{max}}. 
\end{align}
% \begin{align}\label{eqn:todmax_constraint}
%     t_{od}^{\text{max}} = \frac{A_{ub}}{m_1} + \sqrt{\left(\frac{A_{ub}}{m_1}\right)^2+\frac{2}{m_1}\left(V_{\text{th}}\tau + B \right)} \le T_{\text{on}}^{\text{min}}.
% \end{align}

Equations (\ref{eqn:vtrigtau_constraint}), (\ref{eqn:tau_constraint}), and (\ref{eqn:todmax_tonmin}) represent {\em a closed-form expression set for worst-case design} (Design Expression Set).  It is informative to investigate how designs based on this expression set are conservative.  Typically, comparator time constant $\tau$ is chosen based on a particular worst-case interference specification $(\hat{A},\hat{\omega})$ based on (\ref{eqn:vtrigtau_constraint});\footnote{We use the normalized value ($\hat{A}$, $\hat{\omega}$) and $\hat{\tau}$ instead of the actual value ($A_{ub}$, $\omega_l$) and $\tau$
% of the interference amplitude, lower bound on interference frequency and comparator time constant
so that the figures can be used to analyze a more general class of circuits. The normalization procedure is described in (\ref{eqn:def_omega_star}), (\ref{eqn:def_a_star}) and (\ref{eqn:def_g_star}).} however, this particular $\tau$ will guarantee stability for a broad range of interference. Additionally, the transient response of the system can be estimated from the required minimum on time in (\ref{eqn:todmax_tonmin}) and (\ref{eqn:tau_constraint}); however, the actual transient response will most often be faster. 

We compare all the design specifications $(\hat{A},\hat{\omega})$ that result in a particular $\tau$ with the Monte Carlo results of (\ref{eqn:ITlinear}) and (\ref{eqn:forwardpath}).  The Monte Carlo data is generated from the interference over a distribution of $\hat{A}$,  $\hat{\omega}$, and phase using a class of worst-case signals.\footnote{These trapezoidal signals are discussed in Section \ref{section:opd}.}  Figs.~\ref{fig:opd_stab_k_0_3} and \ref{fig:opd_stab_k_0_6} show that (\ref{eqn:vtrigtau_constraint}) results in a large contiguous boundary of stable design specifications. Fig.\,\ref{fig:opd_delay_k_0_6} shows that the designs from (\ref{eqn:tau_constraint}) and (\ref{eqn:todmax_tonmin}) that result in an estimated speed $T_{\text{on}}^{\text{min}}$ nearly match the designs from Monte Carlo.

% shows that the estimate (i.e. lower bound) of the speeds of the system (i.e. minimum on time) are nearly that 

% Fig 36a and b = stability regions
% Fig 36 b = shows optimal designs (64) is inside the stability region
% Fig 36 d->c = the transient estimate is not too conservative


% % Monte Carlo of interference in (\ref{eqn:ITlinear}) and (\ref{eqn:forwardpath}) over a distribution of $\hat{A}$,  $\hat{\omega}$, and phase using a class of worst-case signals.\footnote{These trapezoidal signals are discussed in Section \ref{section:opd}.}

% % Theory Point TP: Square wave signals once they are sampled are inherently trapezoidal, i.e. bandlimited. Sampling is inherently bandlimiting.

% %The interference waveform that we use in the study is a square wave with $50\,\%$ duty ratio, amplitude $A_{ub}$ and fundamental frequency $\omega_l$.
% %It is the limit case of the worst-case interference waveform given the upper bound of amplitude $A_{ub}$ and lower bound of frequency $\omega_l$ \cite{Zhang2015a}. 

% Explaining what a region of bounds means:

% Stable design == that we chose tau for a worst-case interference specification.

% Theorems 6 and 7:
% Assumptions on interference: 
% 1) Lipshitz continuous
% 2) Additive interference
% 3) Bandlimited with no dc component

% Theorems 6:  Upper bound on tau over phase variation (any), bounded amplitude variation, bounded frequency variation (closed interval omega low to omega high)
% $omega_low$ $==>$ in practice $omega_low$ can be chosen as within the bandwidth of the outer loop.

% Monte-Carlo:
% Same assumptions 1,2,3
% Sweep over phase, amplitude, and bounded fundamental frequency range
% bounded frequency range == $omega_low$ to $omega_high$ --> 10x switching frequency
% $W(t,amplitude, phase, fundamental frequency) ==> 50\% square wave$
% Monte-Carlo of a worst-case interference signal

% Fig.36 c and d: Estimate (lower bound) of the speed of the design.  Actual design is faster.  Show that the estimate is not too conservative.  Boundary = 

% We examine the tolerance of this design methodology to a variety of interference by {\bf comparing the theoretical results with Monte Carlo (MC) numerical results.}  Monte Carlo methods can be used for design as well, but there are no provable guarantees on performance and stability.  The results suggest that the designs based on theory are not overly conservative. 

% We compare the design equations in  Theorem\,\ref{theorem:gmax4stability} and Theorem\,\ref{theorem:gmax4overdrivedelay} with a benchmark method --- Monte Carlo (MC) simulation in Fig.\,\ref{fig:opd_stab_delay_comp}.
% The results suggest that the design equations are advantageous in the mathematical rigor, engineering intuition and tiny computational cost by being slightly conservative.

% We use the MC simulation as a baseline because it is expected to be close to the ground truth as a large amount of trials are performed.
% Both methods are performed on the system (\ref{eqn:opd_sys}). The design guide in Theorem\,\ref{theorem:gmax4stability} bounds the nonlinear constraint function (\ref{eqn:ITlinear}) by (\ref{eqn:sc_bd_psi_opd}).
% The MC simulation directly solves the constraint (\ref{eqn:ITlinear}) numerically.
% The optimization problem can be formulated as maximizing the tight sector bounds of the nonlinear function in (\ref{eqn:ITlinear}) with the phase of interference as the decision variables.

% Here we use case studies to show that this design equation is conservative-free.
% In the case study shown in Fig\,\ref{fig:opd_stab_k_0_3} and Fig.\,\ref{fig:opd_stab_k_0_6}, we compare the \emph{stable region} from the design equation in Theorem\,\ref{theorem:gmax4stability} with that from the Monte Carlo simulation. 
% In the case study shown in Fig\,\ref{fig:opd_delay_k_0_3} and Fig.\,\ref{fig:opd_delay_k_0_6}, we compare the \emph{acceptable overdrive delay region} from the design equation in Theorem\,\ref{theorem:gmax4overdrivedelay}  with that from the Monte Carlo simulation.

% The \emph{tolerable region for stability}, as shown in Fig.\,\ref{fig:opd_stab_k_0_3} and \ref{fig:opd_stab_k_0_6}, is defined as the collection of interference types $(\hat{A}, \hat{\omega})$ which don't cause the unstable current-control loop. 
% The \emph{tolerable region for minimum on time}, as shown in Fig.\,\ref{fig:opd_delay_k_0_3} and \ref{fig:opd_delay_k_0_6}, is defined as the collection of interference types $(\hat{A}, \hat{\omega})$ which don't cause the maximum overdrive delay to exceed the minimum on time.
% The tolerable region for stability enlarges with $\hat{\tau}$ whereas that for minimum on time shrinks with $\hat{\tau}$. 
% given a comparator with time constant $\hat{\tau}$,
% For a comparator with time constant $\tau$, the solution set of (\ref{eqn:vtrigtau_constraint}) is the \emph{stable region}.
% As shown in Fig.\,\ref{fig:opd_stab_k_0_3} and \ref{fig:opd_stab_k_0_6}, the stable region enlarges with $\tau$.
% For a comparator with time constant $\tau$, the solution set of (\ref{eqn:todmax_constraint}) is the \emph{acceptable overdrive delay region}. 
% As shown in Fig.\,\ref{fig:opd_delay_k_0_3} and \ref{fig:opd_delay_k_0_6},
% The intersection of tolerable region for stability and that for minimum on time determines the interference which the comparator $\tau$ can condition.

% Given a small $\hat{\tau}$, as shown in Fig.\,\ref{fig:opd_stab_k_0_3} and Fig.\,\ref{fig:opd_delay_k_0_3}, the tolerable region for stability is smaller. This indicates that the instability issue mainly bottlenecks the comparator-overdrive-delay conditioning.
% Given a big $\tau$, as shown in Fig.\,\ref{fig:opd_stab_k_0_6} and Fig.\,\ref{fig:opd_delay_k_0_6}, the tolerable region for minimum on time is smaller. This indicates the long overdrive delay issue mainly bottlenecks the comparator-overdrive-delay conditioning.

% We can imagine that the true tolerable regions are complicated from Fig.\,\ref{fig:opd_stab_delay_comp}.
% The design equations lead to a convex subset in the ground-truth region.
% By using the design equations, We gain the mathematical rigor, engineering intuition and tiny computational cost by being slightly conservative.
% In another word, the comparator design based on design equations sufficiently results in a stable current-control loop from the Monte Carlo simulation.
% The true simulation region is
% The acceptable overdrive delay region


% we realize that we can increase the comparator time constant $\tau$ to enlarge the stable region. 
% However, we can not select $G$ to be arbitrarily small because it causes a huge overdrive delay which is longer than the maximum on-time.
% This restriction imposes a lower bound on $G$. In Fig.\,\ref{fig:opd_stab_k_0_3}, all the propagation delay are shorter than the maximum on-time.
% In Fig.\,\ref{fig:opd_stab_k_0_6}, the stability region in orange is infeasible because the overdrive delay are longer than the maximum on-time. Only the stability region in blue is feasible.
% This observation indicates that there exists a bound on the interference which the comparator overdrive can condition. For the interference outside of that bound, the overdrive delay cannot condition the current-control loop no matter how we tune the time constant $\tau$.

% We \mbox{completely} characterized by two parameters --- the amplitude $A_{ub}$ and fundamental frequency $\omega_l$.
% We consider the triplet of 
% \mbox{transconductance}, amplitude of interference, frequency of
% interference ($G$, $A$, $\omega$) as the \emph{parameter vector}. 
% The set of parameter vector which results in the globally asymptotically stability of current-control loop is denoted by
% \emph{stabilizing parameter set}.
% Figure\,\ref{fig:opd_stab_k_0_3} and Fig.\,\ref{fig:opd_stab_k_0_6} compare a \emph{stabilizing parameter subset} from Theorem\,\ref{theorem:gmax4stability} with that from the numerical results.
% This subset is obtained by fixing the transconductance $G$ and projecting the stabilizing parameter set to the subspace spanned by the amplitude and frequency of interference.

% Figure\,\ref{fig:opd_stab_k_0_3} and Fig.\,\ref{fig:opd_stab_k_0_6} show that the theoretical stability region is a subset of the simulated stability region. 
% We notice that for the interference whose lower bound on frequency is relatively higher than the switching frequency, the stable region from the design equations is very close to the true stable region.
% When the interference whose lower bound on frequency is relatively low compared to the switching frequency, the designer can combine the design equations and Monte Carlo optimization for the less-conservative results (can refer to our toolbox).
\begin{figure*}[ht]
\centering
\subfigure[Stable Designs $(\hat{A}, \hat{\omega})$ with $\hat{\tau} = 0.3$  from: 
\newline({\color{blue}$\blacksquare$})~Monte Carlo; ({\color{red}$\blacksquare$})~Design Expression Set.  
\newline (increase the linewidth by 50\%, 
\newline match the blue/red in matlab, )]{
\includegraphics[width = 0.3\textwidth]{Stability_Comp_k_0_3.pdf}\label{fig:opd_stab_k_0_3}
}
\subfigure[Stable Designs $(\hat{A}, \hat{\omega})$ with $\hat{\tau} = 0.6$ from:
\newline ({\color{blue}$\blacksquare$})~Monte Carlo; ({\color{red}$\blacksquare$})~Design Expression Set.
\newline (increase the linewidth by 50\%, delete the optimal green line, delete the optimal green line)]{
\includegraphics[width = 0.3\textwidth]{Stability_Comp_k_0_6.pdf}\label{fig:opd_stab_k_0_6}
}
% \subfigure[Tolerable region for minimum on time given $\hat{\tau} = 0.3$, $\hat{T}_{\text{on}}^{\text{min}} = 0.3$.]{
%     \includegraphics[width=0.225\textwidth]{Figure/section3/opd/Overdrive_Comp_k_0_3.pdf} 
%     \label{fig:opd_delay_k_0_3}
% }
% % \caption{The stability region from the design equations is inside the stability region from the Monte Carlo simulation.}
\subfigure[Stable Designs $(\hat{A}, \hat{\omega})$ with $\hat{\tau} = 0.6$ and $\hat{T}_{\text{on}}^{\text{min}} = 1$  from: 
\newline({\color{blue}$\blacksquare$})~Monte Carlo; ({\color{green}$\blacksquare$})~Design Expression Set.
\newline(increase the linewidth by 50\%, change red line to green)]{
    \includegraphics[width=0.3\textwidth]{Overdrive_Comp_k_0_6.pdf} 
    \label{fig:opd_delay_k_0_6}
}
\caption{The tolerable regions from the Theorem\,\ref{theorem:gmax4stability} and Theorem\,\ref{theorem:gmax4overdrivedelay} are subsets of that from the Monte Carlo (MC) simulation. % The acceptable overdrive delay region from the design equation (\ref{eqn:todmax_constraint}) is a subset of that from the MC simulation.
}
\label{fig:opd_stab_delay_comp}
\end{figure*}
We define the \emph{normalized interference frequency} as
\begin{align} \label{eqn:def_omega_star}
    \hat{\omega} \triangleq \frac{\omega_l}{\omega_b}, \quad \omega_b \triangleq \frac{2\pi}{T_{\text{on}}},
\end{align}
the \emph{normalized interference amplitude} as
\begin{align} \label{eqn:def_a_star}
    \hat{A} \triangleq \frac{A_{ub}}{A_b}, \quad  A_b \triangleq \frac{A_{ub}}{m_1T_{\text{on}}},
\end{align}
the \emph{normalized comparator time constant} as
\begin{align} \label{eqn:def_g_star}
    \hat{\tau} \triangleq \frac{\tau}{\tau_b}, \quad \tau_b \triangleq\frac{m_1T^2_{\text{on}}}{2V_{\text{trig}}},
\end{align}
and the \emph{normalized minimum on time} as
\begin{align} \label{eqn:def_on_time_star}
    \hat{T}_{\text{\text{on}}}^{\text{min}} \triangleq \frac{T_{\text{\text{on}}}^{\text{min}}}{T_{\text{\text{on}}}}.
\end{align}
The base value for the normalization were chosen to be the operating points in the steady state. For example, $T_{\text{on}}$ represents the on time of the current-control loop in the steady state.

%As shown in Figs.~\ref{fig:copd_nomogram_p1},~\ref{fig:copd_nomogram_p2} and \ref{fig:copd_nomogram_p3}, the $x$\,-\,axis is the normalized interference amplitude and the $y$\,-\,axis is the normalized interference frequency.
%The contour line indicates different lower bound of the time constant of comparator $\hat{\tau}$.

% namely maximum gain $G^*$. We use the reciprocal gain because it is more linear with $A$ and $\omega$ than the gain, hence it makes the interpolation in the nomogram more accurate.

We can acquire more intuition on the stability of the current-control loop with comparator-overdrive-delay conditioning through linearization. 
The linearized model can be expressed as a block diagram in Fig.\;\ref{fig:luresystem} with the linear feedback gain 
\begin{align} \label{eqn:S2}
\psi = \frac{f(T_{\text{on}}) - f(T_{fi})}{T_{\text{on}} - T_{fi}},
\end{align}
where $T_{fi}$ is the steady-state value of (\ref{eqn:final_i_eqn_num_trick}) and $T_{\text{on}}$ is the on time in the steady state.

Interference manifests in the feedback gain $\psi$ as described in Section \ref{current_map_ctrl_perform}.
Negative $\psi$ results in positive feedback and may destabilize the current-control loop.
Larger comparator time constant $\tau$ results in longer delay from $T_{fi}$ to $T_{\text{on}}$.
From (\ref{eqn:S2}), larger $T_{\text{on}} - T_{fi}$ can decrease the amplitude of $\psi$ and stabilize the current-control loop.  However, either positive or negative feedback can result in stable control loop. 

We can visualize the stabilizing effect of comparator-overdrive-delay conditioning through the root locus, which is shown in Fig.\;\ref{fig:lc_copd_cotcm}. We observe that comparator-overdrive-delay for positive feedback in Figs.~\ref{fig:lc_copd_cotcm} (a) and (b) move the location of the worst-case closed-loop pole further to the right, hence improving stability margin.  Likewise, for negative feedback in Figs.~ \ref{fig:lc_copd_cotcm} (c) and (d), the closed-loop pole moves further to the left.  In this way, comparator-overdrive-delay conditioning can guarantee that the closed-loop poles stay inside the unit disk, hence guaranteeing stability.
\begin{figure}
    \centering
    \includegraphics[width=7 cm]{lc_copd_cotcm.pdf}
    \caption{Root locus of the constant off(on)-time current-control loop with the comparator overdrive delay.}
    \label{fig:lc_copd_cotcm}
\end{figure}

We next show the quantitative relationship between interference and the location of closed-loop pole. From (\ref{eqn:filter_lin_sys2}), the closed-loop transfer function is 
\begin{align} % \label{eqn:iltf1} 
     C_2(z) = \frac{\beta }{1-az^{-1}},
\end{align}
where
\begin{align} %\label{eqn:filter_ztransform}
       \beta = \frac{m_1}{m_1 + \psi}, \quad a = \frac{\psi}{m_1 + \psi};
\end{align}
$\psi$ is defined in (\ref{eqn:S2}). Given an interference with amplitude upper bound $A_{ub}$ and frequency lower bound $\omega_l$, $\psi$ is bounded within the range $[\psi_{\text{min}}, \psi_{\text{max}}]$ where
\begin{align}
   \psi_{\text{min}} = \frac{-2m_1}{1 + \sqrt{1 + \frac{1}{\hat{A}^2}(\hat{\tau} - \frac{\hat{A}}{\hat{\omega}})}}, \nonumber \\
    \psi_{\text{max}} = \frac{2m_1}{-1 + \sqrt{1 + \frac{1}{\hat{A}^2}(\hat{\tau} - \frac{\hat{A}}{\hat{\omega}})}}.
\end{align}
The detailed derivations can be found in Appendix\,\ref{proof:gmax4stability}.
For different operating points, the pole $a$ is always real and within the range $[a_{\text{min}},a_{\text{max}}]$ where
\begin{align} \label{eqn:range_pole_sc}
a_{\text{min}} = \frac{\psi_{\text{min}}}{(m_1 + \psi_{\text{min}})}, \quad
a_{\text{max}} = \frac{\psi_{\text{max}}}{(m_1 + \psi_{\text{max}})}.
\end{align}
The condition for small-signal stability is
\begin{align} \label{eqn:stab_pole_sc}
\abs{a_{\text{min}}}<1 , \quad \abs{a_{\text{max}}}<1.
\end{align}
The worst-case settling and overshoot can be obtained from (\ref{eqn:settlecycle1}) and (\ref{eqn:overshoot1}), respectively. 
\begin{figure*}[ht]
\centering
\subfigure[The relationship between the worst-case settling $N_w$ and the time constant $\hat{\tau}$ of the comparator. The frequency of the interference is $\hat{\omega} = 2$. {\color{red}(Need adding the legends)}]{
\includegraphics[width=0.3\textwidth]{opd_settlingtime.pdf} \label{fig:opdr_settlingtime}}
\subfigure[The relationship between the worst-case overshoot $O_w$ and the time constant $\hat{\tau}$ of the comparator. The frequency of the interference is $\hat{\omega} \mbox{= 2}$.{\color{red}(Need adding the legends)}]{
    \includegraphics[width=0.3\textwidth]{opd_overshoot.pdf}
    \label{fig:opdr_overshoot}
}
\subfigure[The relationship between the maximum comparator overdrive delay $t_{od}^{\text{max}}$ and the time constant $\hat{\tau}$ of the comparator. The frequency of the interference is $\hat{\omega} = 2$. {\color{red}(Need adding the legends, in axis $t_{od}$, $\tau$ should be normalized)}]{
    \includegraphics[width=0.3\textwidth]{opd_overdrive_delay.pdf} 
    \label{fig:opdr_overdrive_delay}
}
\caption{The design diagram for comparator overdrive given different interference levels.}
\label{fig:opdr_settling_overshoot}
\end{figure*}
Figures~\ref{fig:opdr_settlingtime}, \ref{fig:opdr_overshoot}, and \ref{fig:opdr_overdrive_delay} show how the settling, overshoot and overdrive delay change with the comparator time constant.
We observe that both the settling and overshoot decrease as comparator time constant $\hat{\tau}$ increases; also, overdrive delay increases as $\hat{\tau}$ increases. These observations match our intuition because the increase in the comparator time constant results in a corresponding increase in the ability of the comparator to attenuate interference; hence, overshoot and settling is smaller. However, with this increase in comparator time constant, overdrive delay is longer, in consequence sacrificing large-signal speed.
% We explain this observation by a simpler related problem of filtering a sinusoidal interference by moving average. The optimal window size should be the integer multiplication of the period of this sinusoidal interference. Any averaging window with larger and smaller size cannot totally eliminate the interference.
% Therefore, as $\hat{\tau}$ increases, a group of local optima appear.
% We select the smallest $\hat{\tau}$ among the local minimums because it results in the shortest overdrive delay. 


% Figures \ref{fig:stabstep} and \ref{fig:unstabstep} demonstrate a simulation verification of the theory. The parameters can be found in Table \ref{table:cotcm_boost_param} and Section \ref{subsection:opddesignguide}.

% \begin{table}[tb]
%     \caption{DESIGN PARAMETERS OF THE CONSTANT OFF-TIME CURRENT-MODE BOOST CONVERTER. {\color{red} no need boost converter data any more}}
%     \label{table:cotcm_boost_param}
%     \centering
%     \begin{tabular}{cccccccccccccc}
%         \toprule
% \textbf{Parameters}&\textbf{Values}&\textbf{Parameters}&\textbf{Values}\\
% \midrule
% $\mathbf{V_{\textbf{in}}}$
% & 12\,V & $\mathbf{L}$ & 6.8$\mu$H\\
% \midrule
% $\mathbf{V_{\textbf{out}}}$
% & 35\,V & $\mathbf{R_{\textbf{sample}}}$
% & 100\,m$\Omega$ \\
% \midrule
% $\mathbf{I_{\textbf{out}}}$ 
% & 0.68\,A & $\mathbf{f_{\textbf{int}}}$
% & 6\,MHz \\
% \midrule
% $\mathbf{T_{\textbf{off}}}$ 
% & 200\,ns & $\mathbf{A_{\textbf{int}}}$
% & 10\,mV \\
% \midrule
% $\mathbf{C}$ & 1 $\mu$F & \, &\, \\
%         \bottomrule
%     \end{tabular}
% \end{table}

% \begin{figure}[ht] 
% \centering
% \subfigure[G = 1 $\times 10^8$ (stable)]{
% \includegraphics[width=8 cm]{Figure/section4/stabcurrentstep.pdf} 
%     \label{fig:stabstep}
% }
% \subfigure[G = 3 $\times 10^8$ (unstable because of the limit cycle)]{
%     \includegraphics[width=8 cm]{Figure/section4/instabcurrentstep.pdf} 
%     \label{fig:unstabstep}
% }
% \caption{Inductor current step response with different comparator overdrive delay.}
% \end{figure}

The analysis in this section can be used for control conditioning fixed-frequency peak current-mode control by substituting $G(z)$ in (\ref{eqn:gzofcotcm}) by (\ref{eqn:fpccplanttf}).
To extend the analysis to the constant on-time control or the fixed-frequency valley current-mode control, we need to substitute $m_1$ by $m_2$ and $T_{\text{on}}$ by $T_{\text{off}}$ in  (\ref{eqn:def_omega_star}) and (\ref{eqn:def_a_star}).

% \begin{figure}
% \begin{minipage}{0.48\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{Figure/section3/opd/nomogram_p1_c.pdf}
%     \caption{The nomogram for choosing the OPD gain by interference amplitude $A_{\text{int}} \in [0,1]$  and frequency $\omega_{\text{int}} \in [0,0.5]$.}
%     \label{fig:mynomogram_p1}
% \end{minipage}
% ~
% \begin{minipage}{0.48\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{Figure/section3/opd/nomogram_p2_c.pdf}
%     \caption{The nomogram for choosing the OPD gain by interference amplitude $A_{\text{int}} \in [0,1]$ and frequency $\omega_{\text{int}} \in [0.5,3]$.}
%     \label{fig:mynomogram_p2}
% \end{minipage}
% \end{figure}
%\subsubsection{Stability Analysis}
% The next Theorem provides us a way to calculate $G_{\text{min}}$.
% \begin{theorem} \label{theorem:gmin4stability}
% To guarantee the OPD to not exceed $T_{\text{on}}$, the $G_{\text{min}}$ is
% \begin{align}
%   G_{\text{min}} = V_{\text{th}}
%   \left( \frac{m_1}{2}T^2_{\text{on}} - A T_{\text{on}} - \frac{2A}{\omega}\right)^{-1}.
% \end{align}
% \end{theorem}
% The proof is shown in Appendix \ref{proof:gmin4stability}. It can be extended to constant on-time current-mode control by substituting $m_1$ by $m_2$.

% We assume $f$ is a periodic signal with bounded amplitude $[A_{\text{min}},A_{\text{max}}]$.


% Then the location of the pole can be bounded by
% \begin{align} \label{SC21}
% a^i_{1_{\text{min}}} =  1 - \frac{1}{1 + \frac{A_{\text{min}}-A_{\text{max}}}{m_1t_{l_{\text{min}}}}} \le a^i_1 \le a^i_{1_{\text{max}}} = 1 - \frac{1}{1 + \frac{A_{\text{max}}-A_{\text{min}}}{m_1t_{l_{\text{min}}}}}
% \end{align}

%\subsubsection{Highlights of this method}
% We conclude that comparator overdrive is an optimal nonlinear filter for a ramp signal in the sense of control conditioning because it does not affect the linearity of static mapping given a ramp signal. 
% This implies that a good conditioning method in the sense of control conditioning may not be a good method in the sens of signal conditioning.

In summary,  comparator-overdrive-delay conditioning can be a powerful control conditioning approach that can be easily implemented. The analog comparator, which is commonly used in peak current-mode control, can directly have a dual-use as an interference attenuator without extra complexity.
Within an integrated circuit, the level of attenuation can be easily chosen by adjusting the tail current.

A step-by-step design guide for comparator-overdrive-delay conditioning is provided in Section \ref{subsection:opddesignguide}.

==> 4_solution_filter.tex <==
\subsection{Low-Pass Filter Conditioning} \label{sec:solution_subsec:lowpassfilter}
The low-pass filter is used in the signal conditioning to \mbox{reduce} the amplitude of the interference signal.
The interference frequency is required to be well above switching frequency.
In this way, the cut-off frequency of low-pass filter can be above switching frequency. 
The interference amplitude can be attenuated without affecting the inductor current ramp.
% From the perspective of control conditioning, the low-pass filter not only reduces the amplitude of the interference signal but also warps the static mapping and introduces a new smooth nonlinearity.
% Therefore, The cut-off frequency of the low-pass filter can be designed to be nearly at or below the switching frequency.
When the time scale of the interference is near or below the switching frequency, the cut-off frequency will be near or below the switching frequency.
Control conditioning not only considers the reduction in the interference amplitude, but also the introduction of a new, but undesirable smooth nonlinearity.
% The difference is control conditioning approach treats the warping effect of ramp intrinsic while signal conditioning approach treats the warping effect of ramp extrinsic.
% Because of this, the control conditioning approach overcomes the limitation that low-pass filter can only deal with the interference whose spectrum is around or below the switching frequency.
% From the control conditioning perspective, you can actually account for the fact that the cut-off frequency is nearly at or below the switching the frequency.
At the same time, the stability and good transient performance is still guaranteed.

Low-pass filter can repair both discontinuity and nonlinearity problem in static mapping.
% Filter can also improve the transient performance of dynamical mapping.
Despite the introduction of an undesirable nonlinearity, the filter repairs discontinuities in the static mapping, and can actually improve the interference\nobreakdash-degraded transient performance of the dynamical mapping by reducing the interference amplitude.

{\color{red}
 interference --> early/late trigger--> event deviation--> deviation in actual current--> defect in static mapping.
 The filter decreases the degree of nonlinearity of static mapping, as shown in Fig.\,\ref{fig:filter_imap_with_inf}.
The early trigger, which is caused by positive interference, can be delayed by filter. The late trigger, which is caused by negative interference, can be advanced by filter.
The filter decreases the degree of nonlinearity of the \red{(make sure if the ideal mapping makes sense?) ideal static mapping}, as shown in Fig.\,\ref{fig:filter_imap_no_inf}.
Therefore, there exists an optimal parameter for filter to perform the control conditioning.
}
% Low-pass filter, the traditional way to tackle against the interference, stabilizes the current-control loop by attenuating the amplitude of interference. However, as shown in Fig.\;\ref{fig:filter1}, the actual inductor current may be distorted. In this section, we develop a theory to optimize the design of the filter.
% \subsubsection{Modeling of the current bluecontroller with low-pass filter}

The current-control loop using constant off-time can be modeled as
% \begin{align}
% i_p[n] &= i_p[n-1] - m_2T_{\text{off}} +m_1t_{\text{on}}[n], \nonumber \\
% i_c [n] &= (i_p[n-1] - m_2T_{\text{off}})(1-e^{-t_{\text{on}}[n]/\tau}) 
%      + \int_0^{t_{\text{on}}[n]} m_1 (1-e^{t/\tau}) dt  \nonumber \\
%      & + i_c [n-1] e^{-T_{\text{off}}/\tau} e^{-t_{\text{on}}[n]/\tau} 
%      + \frac{A \, \text{sin}(\omega  t_{\text{on}}[n]+\varphi)}{\omega \tau}.
% \end{align}
\begin{subequations}
\begin{align} 
    \label{eqn:filter_nonlin_sys} i_p[n] =\,& i_p[n-1] -m_2T_{\text{off}} +m_1\,t_{\text{on}}[n],\\
 %h(t)\bigg_{t=t_{\text{on}}[n]},
    \label{eqn:filter_nonlin_sys_fb} i_c [n] =\,& h_0(t_{\text{on}}[n]) h_0(T_{\text{off}}) i_c[n-1]
    \nonumber \\
    & + \left(i_m(t) u(t) \ast h(t)\right)\bigg\rvert_{t=t_{\text{on}}[n]},
\end{align}
\end{subequations}
where ${\ast}$ is the convolution operator, $h(t)$ is the impulse response function of the low-pass filter, $h_0(t)$ is the zero input response of filter and $u(t)$ is the unit step function.
Equation (\ref{eqn:filter_nonlin_sys_fb}) captures the low-pass filter response.
The $i_m(t)$ represents the current sensor output and filter input.
$i_m(t)$ can be expressed as the additive summation of inductor current on the bottom switch and interference 
\begin{align}
    i_m(t) = i_p[n-1] - m_2T_{\text{off}} + m_1 t + w(t).
\end{align}
% The desired current $I_c$ and actual current $I_p$ at the equilibrium satisfy
% \begin{align} \label{eqn:equic_front}
%     I_c = \frac{\left(\left( I_p -m_2T_{\text{off}} + m_1 \, t + w(t) \right) u(t){\ast}h(t)\right)\bigg\vert_{t=T_{\text{on}}}
%     }{1-q(T_{\text{on}})q(T_{\text{off}})}.
% \end{align}
% \begin{figure}
%     \centering
%     \includegraphics[width=8cm]{filter.pdf}
%     \caption{Comparison of current-sense voltage with/without the interference and with/without the filter. {\color{blue}---} is for the current-sense voltage with interference and without filter. {\color{red}$\cdots$} is for the current-sense voltage with interference and with filter. {\color{green}-\,$\cdot$\,-} is for the current-sense voltage without interference and without filter. {\color{orange}-\,-\,-} is for the current-sense voltage without interference with filter.}
%     \label{fig:filter1}
% \end{figure}
\begin{figure}
    \centering
    \includegraphics[width = 6cm]{filter_imap_with_inf.pdf}
    \caption{Filter shows a weakening effect on the nonlinearity of the static current mapping because it attenuates the interference signal.}
    \label{fig:filter_imap_with_inf}
\end{figure}
\begin{figure}
    \centering
    \includegraphics{filter_imap_no_inf.pdf}
    \caption{Filter shows an enhancing effect on the nonlinearity of the static current mapping because it warps the ramp signal.}
    \label{fig:filter_imap_no_inf}
\end{figure}
% \begin{align}
% \tilde i_p[n] &= \tilde i_p[n-1]  +m_1 \tilde t_{\text{on}}[n], \nonumber \\
% \tilde i_c [n] &=  (1-e^{-T_{\text{on}}/\tau}) \tilde i_p[n-1]+ \frac{(I_p - m_2T_{\text{off}})}{\tau}e^{-T_{\text{on}}/\tau} \tilde t_{\text{on}}[n] + m_1 (1-e^{-T_{\text{on}}/\tau}) \tilde t_{\text{on}}[n]   \nonumber \\
%         &+  e^{-T}/\tau \tilde i_c [n-1] -\frac{I_c e^{-T_{\text{off}}/\tau}}{\tau} + e^{-T_{\text{on}}}/\tau \tilde t_{\text{on}}[n]
%         + \frac{A\, \text{cos}(\omega T_{\text{on}}+\varphi)}{\tau} \tilde t_{\text{on}}[n].'''''''''
% \end{align}
% \begin{align} \label{eqn:filter_lin_sys2}
% \tilde i_p[n] = \; & \tilde i_p[n-1]  +m_1 \, \tilde t_{\text{on}}[n], \nonumber \\
% \tilde i_c [n] = \; & b \,\tilde i_c [n-1] +  c_1 \, \tilde i_p [n] +  c_2 \, \tilde t_{\text{on}}[n],
% \end{align}

% \begin{align} \label{eqn:prarameterszdomain}
%     &b = e^{-\frac{T}{\tau}}, \quad c_1 = u(t) {\ast} h(t)\bigg\rvert_{t = T_{\text{on}}} = 1 - e^{-T_{\text{on}}/\tau}, \quad d = e^{-T_{\text{on}}/\tau}, \nonumber \\
%     & c_2 = \left( -\frac{e^{-T/\tau}}{\tau} I_c + I_v\, h(t) + m_1 u(t){\ast} h(t) + A \, \omega\,  \text{cos}(\omega  t+\varphi)\,u(t) {\ast} h(t) + A\,\text{sin}\,\varphi\,h(t) \right)\bigg\rvert_{t = T_{\text{on}}}.
% \end{align}
% where we denote $e^{-T/\tau}$ by $c$ and use $t$ as a shorthand of $T_{\text{on}}$.\\
% The detailed derivations of  (\ref{eqn:prarameterszdomain}) are provided in (\ref{eqn:conv_eq1} -- \ref{eqn:conv_eq4}) of Appendix \ref{sec:proofoptsc}.
% \begin{align}
%      \frac{\text{d}}{\text{d} t} [m_1t\, u(t){\ast}h(t)] &= m_1 u(t){\ast}h(t),  \\
%      \frac{\text{d}}{\text{d} t} [A \, \text{sin} (\omega t+\varphi)\, u(t){\ast}h(t)] &= A\, \omega\, \text{cos}(\omega  t+\varphi) u(t) {\ast} h(t) + A \,\text{sin}\,\varphi\, h(t), \\
%      m_1t\, u(t){\ast}h(t) &= m_1 \left( t + (e^{-t/\tau}-1)\tau \right) u(t),  \\
%      \, \text{sin} (\omega t+\varphi)\, u(t){\ast}h(t) &= \frac{\omega \tau \text{cos}\, \varphi - \text{sin}\varphi}{1 + \omega^2 \tau^2} e^{-\frac{t}{\tau}}u(t) + \frac{\text{sin}(\omega t+\varphi)-\omega\tau \text{cos}(\omega t + \varphi)}{1 + \omega^2 \tau^2}u(t).
% \end{align}
\begin{figure}[ht]        
\centering
\includegraphics[width=8 cm]{filter_fb.pdf}
\caption{Block diagram of the constant on-time/fixed-frequency peak current control loop with the filter.} \label{fig:filteredccb_fb}
\end{figure}

\begin{figure}[ht] 
\centering
\includegraphics[width=8 cm]{filter_cotcm.pdf}
\caption{Root locus without (left)/with (right) filter. {\color{green}---} is for the negative feedback; {\color{blue} -\,-\,-} is for the positive feedback. Modeling of the current-control loop with filter. The block is used in the constant on(off)-time control. {\color{red} (need to update)}}
\label{fig:filter_cotcm}
\end{figure}

We exemplify this idea by a first-order low-pass filter with the impulse response function $h(t) = (e^{(-t/\tau)}/\tau)\,u(t)$ and $h_0(t) = e^{(-t/\tau)}$ where $\tau$ represents the time constant.
% We assume that the cut-off frequency of filter is much smaller than the frequency of the interference function $w(t)$
% \begin{align} \label{eqn:timescaleassumption}
%     \omega_l \tau \gg 1,
% \end{align}
We denote the lower bound of the frequency of interference by $\omega_l$.
The continuous static mapping is a prerequisite for the stability analysis. Theorem\,\ref{theorem:taomin4continuity} provides a sufficient condition for the filter to guarantee the continuous static mapping. As long as the time constant satisfies Theorem\,\ref{theorem:taomin4continuity}, the static mapping is continuous.
\begin{theorem} \label{theorem:taomin4continuity}
A current-control loop using constant off-time has minimum on time $T^{\text{min}}_{\text{on}}$ and off time $T_{\text{off}}$. The time constant of the first-order low-pass filter is $\tau$. The interference $w(t)$ satisfy Definition\,\ref{def:inteference}.
The condition for $\tau$ to guarantee the continuous static mapping is
\begin{align} % \label{thoerem:filterstab}
 \frac{\hat{A}_{ub}}{(1-d)\hat{\tau}}\left( 1 + \frac{d}{\sqrt{1 + (2\pi \hat{\omega}_l \hat{\tau})^2}}\right) + \frac{b\hat{I}_{\text{max}}}{(1-d)\hat{\tau}} < 1,
\end{align}
where
\begin{align}
    % k_0 & = \frac{b(1 + \hat{\tau} d -\hat{\tau})}{(1-b)(1-d)\hat{\tau}}, \quad k_1 = \frac{1}{\hat{\tau}(1-d)},
    % \hat{\omega}_l & = \frac{\omega_l}{\omega_n}, \quad
    % \omega_n = \frac{2\pi}{T^{\text{min}}_{\text{on}}}, \quad \hat{I}_{\text{max}} = \frac{I_{\text{max}}}{m_1T^{\text{min}}_{\text{on}}}, \quad
    % \hat{\tau} = \frac{\tau}{T^{\text{min}}_{\text{on}}}, \nonumber \\
    %  T & = T^{\text{min}}_{\text{on}} + T_{\text{off}}, \quad b = e^{-\frac{T}{\tau}}, \quad d = e^{-\frac{T^{\text{min}}_{\text{on}}}{\tau}} \nonumber \\
    %  \hat{A}_{ub} & = \frac{A_{ub}}{m_1T^{\text{min}}_{\text{on}}}.
    \hat{T}^{\text{min}} &= \hat{T}^{\text{min}}_{\text{on}} + 1, \quad
    b = e^{-\frac{\hat{T}^{\text{min}}}{\hat{\tau}}}, \quad d = e^{-\frac{\hat{T}^{\text{min}}_{\text{on}}}{\hat{\tau}}}, \quad \hat{\tau} = \frac{\tau}{T_{\text{on}}}, \nonumber \\ 
    \hat{A}_{ub} &= \frac{A_{ub}}{m_1T_{\text{on}}}, \quad
    \hat{I}_{\text{max}} = \frac{I_{\text{max}}}{m_1T_{\text{on}}},\quad 
    \hat{\omega}_l = \frac{\omega_l T_{\text{on}}}{2\pi}.
\end{align}
\end{theorem}
The proof can be found in Appendix \ref{sec:proof_filter_cont}.
$\hat{\tau}$ can be interpreted as the \emph{normalized time constant}. The $\hat{\tau}$ will be used in the design of the filter in Section \ref{sec:hardwaredesignguide}.
$\hat{T}^{\text{min}}$, $\hat{T}^{\text{min}}_{\text{on}}$, 
$\hat{A}_{ub}$, $\hat{I}_{\text{max}}$, $\hat{\omega}_l$ can be interpreted as the normalized minimum switching period, minimum on time, interference amplitude, maximum inductor current and lower bound on the interference, respectively.

% we can simplify (\ref{eqn:prarameterszdomain}) as
% \begin{align} \label{eqn:prarameterszdomain_simplified} 
%     c_1 = 1 - e^{-\frac{T_{\text{on}}}{\tau}} \quad c_2 =  -\frac{e^{-\frac{T}{\tau}}}{\tau}\,I_c + \frac{e^{-\frac{T_{\text{on}}}{\tau}}}{\tau}\,I_v + \frac{w(T_{\text{on}})}{\tau}.
% \end{align}
% From (\ref{eqn:prarameterszdomain}) to (\ref{eqn:prarameterszdomain_simplified}), we use the following equations:
% \begin{align} 
%     \label{eqn:uhconv} u(t){\ast}h(t) &= \left(1 -e^{-\frac{t}{\tau}}\right)u(t) = (1 - d)u(t), \\
%     \label{eqn:sinapprox} A\,\omega\, \text{cos}(\omega  t+\varphi)\,u(t) {\ast} h(t) + A\,\text{sin}\,\varphi\, h(t) &=  \frac{A \,\omega \,\text{sin}(\omega t + \varphi + \delta)}{\sqrt{1+\omega^2\tau^2}} - \frac{A\, \omega \,\text{sin}( \varphi + \delta)}{\sqrt{1+\omega^2\tau^2}} e^{-\frac{t}{\tau}} + \frac{A\, \text{sin} \,\varphi}{\tau} e^{-\frac{t}{\tau}} \nonumber \\
%      & \approx \frac{A\, \text{sin}(\omega t + \varphi + \delta)}{\tau} - \frac{A\, \text{cos}( \varphi + \frac{\delta}{2})\, \text{sin} (\frac{\delta}{2})}{\tau}\, e^{-\frac{t}{\tau}}  \nonumber \\
%      &\approx \frac{A\,\text{sin}(\omega t + \varphi)}{\tau},
% \end{align}
% where $\delta = \text{tan}^{-1}(1/(\omega \tau))$. (\ref{eqn:sinapprox}) utilize the assumption (\ref{eqn:timescaleassumption}).
% \begin{align}
%       \frac{\text{d}}{\text{d} t} [f_1(t){\ast}f_2(t)] = \frac{\text{d} f_1(t)}{\text{d} t}{\ast}f_2(t) = f_1(t) {\ast} \frac{\text{d}f_2(t)}{\text{d} t}.
% \end{align}
% The equilibrium point $I_c$ can be derived by
% \begin{align}
%     I_c = \frac{m_1(T_{\text{on}}+\tau e^{-T_{\text{on}}/\tau}-\tau)+ \frac{A \, \text{sin}(\omega  T_{\text{on}}+\varphi)}{\omega \tau}
%     +  (I_p - m_2T_{\text{off}}) 
%     \left(1-e^{-T_{\text{on}}/\tau} \right)
%     }{\left(1-e^{-(T_\text{on}+T_{\text{off}})/\tau}\right)}
% \end{align}

From the requirement of continuity, we examine how the filter affects the stability of the current-control loop.
Theorem \ref{theorem:taomin4stability} provides a sufficient condition for stability. If $\tau$ satisfies the condition, the global asymptotic stability is guaranteed.
% We show that our sufficient condition is very close to the sufficient and necessary condition. This means that the range of $\tau$ calculated from our sufficient condition is not too conservative.
This theoretical bound for $\tau$ depends on the maximum inductor current $I_{\text{max}}$, minimum on time $T^{\text{min}}_{\text{on}}$ and the interference.
% Given the appropriately worst-case choice of $I_p$ and $I_c$, the sufficient bound is sufficient and necessary.
%It is an affine function of the amplitude of interference.
% close?? sufficient and necessary--tight bound; claim is that the sufficient is tight also?
\begin{theorem} \label{theorem:taomin4stability}
A current-control loop using constant off-time has a minimum on time $T_{\text{on}}^{\text{min}}$ and fixed off time $T_{\text{off}}$. The time constant of the first-order low-pass filter is $\tau$. The interference $w(t)$ satisfies Definition\,\ref{def:inteference}.
The bound for $\tau$ to guarantee the global asymptotic stability of the current-control loop is
\begin{align} %\label{thoerem:filterstab}
 k_0\frac{1}{\hat{\tau}} + k_1 \frac{\hat{A}_{ub}}{\hat{\tau}}+ k_2 \frac{\hat{A}_{ub}}{\hat{\tau}\sqrt{1 + (2\pi\hat{\omega}_l\hat{\tau})^2} } < \frac{1}{2},
\end{align}
and
\begin{align} %\label{thoerem:filterstab}
 k_3 \frac{\hat{I}_{\text{max}}}{\hat{\tau}} + \frac{\hat{A}_{ub}}{\hat{\tau}} + \frac{\hat{A}_{ub}}{\hat{\tau}\sqrt{1 + (2\pi\hat{\omega}_l\hat{\tau})^2}} < \frac{1}{2},
\end{align}
where
% \begin{align}
%     k_0 & = \frac{d(1 + \hat{\tau} d -\hat{\tau})}{(1-d)^2}, \quad k_1 = \frac{1}{(1-d)}, \; T^{\text{min}} = T^{\text{min}}_{\text{on}} + T_{\text{off}}, \nonumber \\
%     b & = e^{-\frac{T^{\text{min}}}{\tau}}, \quad d = e^{-\frac{T^{\text{min}}_{\text{on}}}{\tau}}, \quad \hat{\tau} = \frac{\tau}{T^{\text{min}}_{\text{on}}}, \quad \hat{A}_{ub} = \frac{A_{ub}}{m_1T^{\text{min}}_{\text{on}}}, \nonumber \\
%     k_2 & = 1 + \frac{(1+d)d}{(1-d)^2}, \quad k_3 = \frac{d-b}{(1-d)^2}, \quad \hat{I}_{\text{max}} = \frac{I_{\text{max}}}{m_1T^{\text{min}}_{\text{on}}}, \nonumber \\
%     \hat{\omega}_l & = \frac{\omega_l}{\omega_n}, \quad
%     \omega_n = \frac{2\pi}{T^{\text{min}}_{\text{on}}}.
% \end{align}
\begin{align}
    k_0 & = \frac{d(\hat{T}_{\text{on}}^{\text{min}} + \hat{\tau} d -\hat{\tau})}{(1-d)^2}, \quad k_1 = \frac{1}{(1-d)}, \; \hat{T}^{\text{min}} = \hat{T}^{\text{min}}_{\text{on}} + 1, \nonumber \\
    b & = e^{-\frac{\hat{T}^{\text{min}}}{\hat{\tau}}}, \quad d = e^{-\frac{\hat{T}^{\text{min}}_{\text{on}}}{\hat{\tau}}}, \quad \hat{\tau} = \frac{\tau}{T_{\text{on}}}, \quad \hat{A}_{ub} = \frac{A_{ub}}{m_1T_{\text{on}}}, \nonumber \\
    k_2 & = 1 + \frac{(1+d)d}{(1-d)^2}, \quad k_3 = \frac{d-b}{(1-d)^2}, \quad \hat{I}_{\text{max}} = \frac{I_{\text{max}}}{m_1T_{\text{on}}}, \nonumber \\
    \hat{\omega}_l & = \frac{\omega_l T_{\text{on}}}{2\pi}.
\end{align}
\end{theorem}
The proof can be found in the Appendix \ref{proof:taomin4stability}. 

do not have continuous deformation in psi!  why is the case?  because you cannot find attributes for the interference that enforce continuous deformation in psi.

interference: 
1) continuous phase of something periodic -- highly narrow class

T and psi are smooth nonlinearities.


Find worst-case nonlinearity in QS mapping from worst-case frequency and worst-case amplitude.

Does the worst case QS nonlinearity correspond to the worst-case slope in psi?

\red{if the design for control performance is based on small signal, then for all ic has to be small signal stable. you need to restrict psi and/or G(z) so the small signal stability for all ic is enforced.  wide-sense small signal stable and large stable at the same time.
(1) choose G(z) so it is stable for all psi'
(2) step 1: G(z) is not conditionally stable over psi'
(3) step 2: can check that it is stable for max psi'}

We can get more intuition on the stability by linearization. 
At the operating point determined by the peak inductor current command $I_c$, the actual peak inductor current $I_p$, the actual valley inductor current $I_v$, at on time $T_{\text{on}}$, we linearize the system (\ref{eqn:filter_nonlin_sys}) and (\ref{eqn:filter_nonlin_sys_fb}) as
\begin{align} \label{eqn:filter_lin_sys2}
\tilde i_p[n] = \; & \tilde i_p[n-1]  +m_1 \, \tilde t_{\text{on}}[n], \nonumber \\
\tilde i_c [n] = \; & q(T_{\text{on}}) q(T_{\text{off}}) \,\tilde i_c [n-1] +  c_1 \, \tilde i_p [n] +  c_2 \, \tilde t_{\text{on}}[n],
\end{align}
where 
\begin{align} \label{eqn:prarameterszdomain}
    c_1 = &  u(t) {\ast} h(t)\bigg\rvert_{t = T_{\text{on}}} \nonumber \\
    c_2 = & -\frac{d\,q\,(t)}{d\,t}\bigg\rvert_{t = T_{\text{on}}} q(T_{\text{off}})I_c + h(T_{\text{on}})I_v \nonumber \\
    & + \frac{d\,w(t)u(t){\ast}h(t)}{d\,t} \bigg\rvert_{t = T_{\text{on}}}.
\end{align}
The system (\ref{eqn:filter_lin_sys2}) are represented in the block diagram in Fig.\;\ref{fig:filteredccb_fb}. 
% \begin{figure}
%     \centering
%     \includegraphics[width = 8cm]{filter_fb.pdf}
%     \caption{Block diagram representation of the current-control loop of PCC with filter}
%     \label{fig:filteredccb_fb}
% \end{figure}
The plant $G$ follows (\ref{eqn:gzofcotcm}).
An extra gain block $K$ is introduced as
\begin{align}
K = \frac{1}{1-e^{-\frac{T_{\text{on}}}{\tau}}}.
\end{align}
An extra pole-zero pair is introduced as
\begin{align}
    P(z) = 1 - e^{-\frac{T}{\tau}}\,z^{-1}.
\end{align}
The effect of interference is shown in the feedback path $\psi_1$ in Fig.\,\ref{fig:filter_cotcm}
\begin{align}
    %  \psi_1 = \frac{w(T_{\text{on}})}{\tau} - \frac{e^{-\frac{T_{\text{on}}}{\tau}}}{\tau}\int_{-\infty}^{+\infty} \frac{W(\omega)}{j\omega}\,d\omega.
    \psi_1 & = \int_{-\infty}^{+\infty} \frac{j\omega W(\omega) e^{j\omega T_{\text{on}}}}{1 + j \omega \tau}\,d\omega - \frac{e^{-\frac{T_{\text{on}}}{\tau}}}{\tau}\int_{-\infty}^{+\infty} \frac{W(\omega)}{1+j\omega \tau}\,d\omega.
\end{align}
The negative $\psi_1$ can result in the positive feedback and destabilize the current-control loop.
The larger the filter time constant $\tau$ is, the better the filter can attenuate the interference. 
We observe there is an another feedback path $\psi_2$ in Fig.\,\ref{fig:filter_cotcm}, which is derived from the static mapping
\begin{align}
     \psi_2 = - \frac{e^{-\frac{T}{\tau}}}{\tau}I_c + \frac{e^{-\frac{T_{\text{on}}}{\tau}}}{\tau}I_v.
\end{align}
This feedback path is a function of the actual current $I_p$ and inductor current ripple $m_2T_{\text{off}}$. 
% {\color{red}
% earlier section we said that the slope was separable in the static mapping because it did not affect the stability of the current loop. ---> only true for the ideal static mapping
% control conditioning -- now slope matters-->  matters for non-ideal static mapping.
% }
A large $I_p$ or small $m_2T_{\text{off}}$ can result in positive $\psi_2$.
The positive $\psi_2$ means a negative feedback path.
It can partially cancel out the positive feedback path in $\psi_1$. It is worth noting that $\psi_2$ is the result of the trapezoidal shape of the current sensor waveform.

We visualize the effect of filter on the stability of current\nobreakdash-control loop through the root locus.
$P(z)$ in Fig.\;\ref{fig:filteredccb_fb} is outside of the loop, hence is not included in the root locus. 
% Moreover, in the worst case, the valley current $I_p-m_2T_{\text{off}}$ is so small that the effect of $\psi_2$ is much smaller than $\psi_1$. 
We collapse $\psi_1$ and $\psi_2$ in the root locus as a single gain.
The root locus of current-control loop is shown in Fig.~\ref{fig:filter_cotcm}. 
We observe that comparator-overdrive-delay for positive feedback in Figs.~\ref{fig:filter_cotcm} (a) and (b) move the location of the worst-case closed-loop pole further to the right, hence improving stability margin.  Likewise, for negative feedback in Figs.~\ref{fig:filter_cotcm} (c) and (d), the closed-loop pole moves further to the left. 
In this way, the filter guarantees the closed-loop poles to always stay inside the unit disk. Therefore the stability is guaranteed.

% Figure\,\ref{fig:filter3Dstab} and Fig.\,\ref{fig:filter2Dstab} compares the 
% sufficient bound on $\hat{\tau}$ in Theorem\,\ref{theorem:taomin4stability}  with the switching-circuit simulation.
% In the simulation, we assume that the interference has only one frequency component.
% Hence the interference can be completely characterized by the amplitude and frequency.
% We sweep the amplitude of interference, frequency of interference and time constant.
% The combination of these three variables which results in the stable current-control loop is annotated in Fig\,\ref{fig:filter3Dstab}.
% Figure\,\ref{fig:filter2Dstab} provides a cross-sectional view of Fig\,\ref{fig:filter3Dstab}.
% % We want to remark three reasons of having this theorem. 
% From Fig.\,\ref{fig:filter2Dstab}, we observe that given the interference, any $\tau$ within the bound from Theorem \ref{theorem:taomin4stability} results in a stable current-control loop in simulation.
% The bound on $\tau$ in simulation is a littler bit larger than the bound in Theorem \ref{theorem:taomin4stability} can be due to two reasons: 1) the Theorem \ref{theorem:taomin4stability} assumes $\omega\tau \gg 1$ 2) the Theorem \ref{theorem:taomin4stability} can guarantee the stability for arbitrary $I_c$ and $I_p$. The simulation result, however, is in specific $I_c$ and $I_p$.

% As shown in Fig\,\ref{fig:filter2Dstab}, given a low-pass filter with time constant$\tau$, the bound on the interference which does not destabilize the current-control loop is always a rectangle. 
% This is because Theorem \ref{theorem:taomin4stability} is a linear function with amplitude and irrelavant with frequency.
% The design based on the stable region from Theorem \ref{theorem:taomin4stability} is more robust to the uncertainties of the amplitude and frequency of interference. This design only requires an estimation on the upper bound of the amplitude of interference. Hence any negative error on the amplitude and any error on the frequency do not cause instability problem. However, the design based on the simulated stable region have low tolerance on the frequency uncertainty of the interference. As shown in Fig.\,\ref{fig:filter2Dstab}, although a filter with $\hat{\tau} = 0.75$ can stabilize a current-control block interfered by a signal with $\hat{A}$ of 0.21 and $\hat{\omega}$ of 1.25, another interference with same amplitude but $\hat{\omega}$ of 1.75 may destabilize the system. This largely decreases the robustness of the system and is not recommended in the practical design. 
% \begin{figure}[ht]
% \centering
% \subfigure[Stable region, unstable region and the boundary in the space of $\hat{A}$, $\hat{\omega}$ and $\hat{\tau}$.]{
% \includegraphics[width=6 cm]{filter_3D_stability_high_resolution.pdf}\label{fig:filter3Dstab}
% }
% \subfigure[A sectional view of Fig. \ref{fig:filter3Dstab} on the plane $\hat{\tau} = 0.75$.]{
%     \includegraphics[width=6 cm]{filter_2D_stability.pdf} 
%     \label{fig:filter2Dstab}
% }
% \caption{The stable region predicted by Theorem 6 is a subset of the simulated stable region.}
% %\label{fig:subfigureExample}
% \end{figure}

% \subsubsection{Transient Performance Analysis}
We next show the quantitative relationship between the interference and location of closed-loop pole. From (\ref{eqn:filter_lin_sys2}), the closed-loop transfer function is 
% \begin{align} \label{iltf1}
% C_2(z) = \frac{\beta (1-b^{i}_1  z^{-1})}{1-a^{i}_1  z^{-1}}
% \end{align}
% \begin{align}
%     a_1^i &= 1 - \frac{m_1(1-e^{-T_{\text{on}}/\tau})}{m_1(1-e^{-T_{\text{on}}/\tau}) + (I_p - m_2T_{\text{off}} - I_c e^{-T_{\text{off}}/\tau}) \frac{e^{-T_{\text{on}}/\tau}}{\tau} + \frac{A\, \text{cos}(\omega T_{\text{on}}+\varphi)}{\tau}}, \nonumber \\
%     b^{i}_1 & =  e^{-T/\tau},  \nonumber \\
%     \beta & = \frac{m_1}{m_1(1-e^{-T_{\text{on}}/\tau}) + \left(I_p - m_2T_{\text{off}} - I_c  e^{-T_{\text{off}}/\tau}\right) \frac{e^{-T_{\text{on}}/\tau}}{\tau} + \frac{A\, \text{cos}(\omega T_{\text{on}}+\varphi)}{\tau}}.
% \end{align}
\begin{align}
     \label{eqn:iltf1} C_2(z) = \frac{\beta (1-b  z^{-1})}{1-a  z^{-1}}
\end{align}
where
\begin{align} %\label{eqn:filter_ztransform}
    a & = 1 - \frac{m_1}{m_1 +  \frac{\psi_1 + \psi_2}{1-d}},
    % a & = 1 - \beta, \quad \beta = \frac{m_1}{s}, 
    \quad b = e^{-\frac{T}{\tau}}, \quad d = e^{-\frac{T_{\text{on}}}{\tau}}, \nonumber \\
    % s & = m_1 +  \frac{\psi_1 + \psi_2}{1-d}, \nonumber \\
    \psi_1 & = \int_{-\infty}^{+\infty} \frac{j\omega W(\omega) e^{j\omega T_{\text{on}}}}{1 + j \omega \tau}\,d\omega - \frac{e^{-\frac{T_{\text{on}}}{\tau}}}{\tau}\int_{-\infty}^{+\infty} \frac{W(\omega)}{1+j\omega \tau}\,d\omega
     \nonumber \\
     \psi_2 & = - \frac{e^{-\frac{T}{\tau}}}{\tau}I_c + \frac{e^{-\frac{T_{\text{on}}}{\tau}}}{\tau}I_v.
%    \label{eqn:transzparam}
\end{align}
% From (\ref{eqn:filter_nonlin_sys}) to (\ref{eqn:filter_lin_sys2}), we use the following algebraic deformation,
% \begin{align} 
%     \label{eqn:uhconv} u(t){\ast}h(t) &= \left(1 -e^{-\frac{t}{\tau}}\right)u(t) = (1 - d)u(t), \\
%     \label{eqn:sinapprox} A\,\omega\, \text{cos}(\omega  t+\varphi) u(t) {\ast} h(t) + A\,\text{sin}\varphi h(t) &=  \frac{A \,\omega \,\text{sin}(\omega t + \varphi + \delta)}{\sqrt{1+\omega^2\tau^2}} - \frac{A\, \omega \,\text{sin}( \varphi + \delta)}{\sqrt{1+\omega^2\tau^2}} e^{-\frac{t}{\tau}} + \frac{A\, \text{sin} \varphi}{\tau} e^{-\frac{t}{\tau}} \nonumber \\
%      & \approx \frac{A\, \text{sin}(\omega t + \varphi + \delta)}{\tau} - \frac{A\, \text{cos}( \varphi + \frac{\delta}{2})\, \text{sin} (\frac{\delta}{2})}{\tau}\, e^{-\frac{t}{\tau}}  \nonumber \\
%      &\approx \frac{A\,\text{sin}(\omega t + \varphi)}{\tau},
% \end{align}
% where $\delta = \text{tan}^{-1}(1/\omega \tau)$. Equation (\ref{eqn:sinapprox}) utilize the assumption that $\omega \tau >> 2 \pi$ and $\delta \rightarrow 0$.
% \begin{align}
%     s_1 &= m_1 (1-e^{-T_{\text{on}}/\tau}) + \frac{A sin(2\pi f t+\phi(f))}{\tau +1/2 \pi f} + \frac{(I_p - m_2T_{\text{off}}-I_c e^{-T_{\text{off}}/\tau})}{\tau}e^{-T_{\text{on}}/\tau} \\
%     \gamma & = 1 - e^{-\frac{T_{\text{on}}}{\tau}} \quad
%     a  = \frac{(I_p - m_2T_{\text{off}}-I_c e^{-T_{\text{off}}/\tau})}{\tau}e^{-T_{\text{on}}/\tau} \quad  b^{i}_1  =  e^{-T/\tau}
% % \end{align}
% Therefore, in $z$-domain, as shown in Fig.  \ref{fig:filter2}, the filter shrinks the poles which were outside of the unit disk into the unit disk. 

We use the settling and overshoot metrics in (\ref{eqn:settlecycle1}) and (\ref{eqn:overshoot1}), respectively, to quantitatively illustrate the relationship between these metrics and the pole locations.  For different operating points, the pole $a$ is within the range $[a_{\text{min}},a_{\text{max}}]$.
We observe that a small $\tau$ does not provide enough attenuation on the interference whereas a too-high $\tau$ distorts the original current ramp. 
Another observation is that a big $\tau$ slows down the zero in (\ref{eqn:iltf1}). A slow zero causes the long-tail settling and overshoot problem in transient response. 
%So there exists a feasible interval $[\tau_{\text{min}}, \tau_{\text{max}}]$ for selecting $\tau$.
% such that for all $\tau \in [\tau_{\text{min}}, \tau_{\text{max}}]$, all the poles of the current-control loop can stay inside the unit disk.
Figure\,\ref{fig:filter_settlingtime} and Fig.\,\ref{fig:filter_overshoot} show how the settling and overshoot change with the time constant. We fix the interference frequency at two times the switching frequency \footnote{For the constant on(off)-time operation, this means the reciprocal of on(off) time, i.e. the fastest switching frequency.} and vary the interference amplitude.
The theoretical relations are represented by the dotted line and the simulated relations are represented by the solid line. 
% The assumption (\ref{eqn:timescaleassumption}) is plotted as the dot-dash line. The half space on the right side of the dot-dash line satisfies the assumption.
We observe that the theoretical curves perfectly match the simulation curves. 
% It is worthwhile to mention that even on the left side of the dot-dash line where the assumption (\ref{eqn:timescaleassumption}) breaks, the theoretical curves can still provide a decent estimation on the settling and overshoot.

The settling first decreases with the time constant $\hat{\tau}$ because the filter attenuates the interference. However, the filter also distorts the original current ramp. With the increase of $\hat{\tau}$, this distortion effect becomes more severe, hence the settling starts to increase with $\hat{\tau}$. Similarly, the overshoot decreases first with $\hat{\tau}$ because the interference is suppressed. However, the filter also introduces a zero in the transfer function (\ref{eqn:iltf1}). This zero becomes slower and causes large overshoot as $\hat{\tau}$ increases. 

In conclusion, the important take-away messages for designers are: 1) there exists the optimal $\hat{\tau}$ to minimize overshoot and settling; 2) the optimal $\hat{\tau}$ increases as the amplitude of interference increases, which is supported by our design diagram. 
% 3) the optimal $\hat{\tau}$ does not change as the frequency of interference changes, which is supported by our theory. 
The step-by-step design guide for filter is shown in Section \ref{subsection:lpf}.
\begin{figure}[ht]
\centering
\subfigure[The worst-case settling $N_w$ decreases first and then increases with the time constant $\hat{\tau}$ of the filter. The interference frequency $\hat{\omega} = 2$.]{
\includegraphics[width=6 cm]{Filterdesign_settlingtime.pdf} \label{fig:filter_settlingtime}
}
\subfigure[The worst-case overshoot $O_w$ decreases first and then increases with the time constant $\hat{\tau}$ of the filter. The interference frequency $\hat{\omega}= 2$.]{
    \includegraphics[width=6 cm]{Filterdesign_overshoot.pdf} 
    \label{fig:filter_overshoot}
}
\caption{The design diagram for filter given different interference levels. The theoretical curves which are represented by the dotted line matches the simulated curves, which are represented by the solid line.}
%\label{fig:subfigureExample}
\end{figure}

% \subsubsection{Analysis on Constant On-time current-control loop}
To extend the analysis to the constant on-time current\nobreakdash-control loop, $G(z)$ is changed to
\begin{align}
    G(z) = \frac{1-z^{-1}}{m_2},
\end{align}
and $\psi_2$ is changed to
 \begin{align}
     \psi_2 = -\frac{d}{\tau}I_p - \frac{b}{\tau}I_c.
 \end{align}
Note that $\psi_2<0$, hence the feedback path $\psi_2$ is a pure positive feedback and it always shrinks the stability margin. Therefore, the filter helps more on the constant off-time control than the constant on-time control. For designers who use the filter in the constant on-time control, the author recommends that it is better to make the time constant of filter faster than the switching period to avoid the bad effect of the  $\psi_2$ feedback path. The simplified root locus of current-control loop is the same as Fig.\;\ref{fig:filter_cotcm}.

% \subsubsection{Analysis on Fixed-frequency current-control loop}
The analysis method can be extended to the fixed-frequency peak current-mode control by substituting $G(z)$ by (\ref{eqn:fpccplanttf}) and substituting the feedback path $\psi_2$ by
\begin{align}
     \psi_2 = \frac{d}{\tau}I_v - \frac{b}{\tau}I_c(1 - z^{-1}).
\end{align}
%We take the fixed-frequency peak current-mode control as an example. 
% We substitute the (\ref{eqn:filter_nonlin_sys}) by (\ref{eqn:ffpccip}) and substitute (\ref{eqn:filter_nonlin_sys_fb}) by 
% \begin{align}
%   i_c [n] &= 
%   e^{-\frac{t_{\text{on}}[n]}{\tau}}
%   e^{-\frac{T_{\text{off}}[n-1]}{\tau}} i_c[n-1] + \left(i_v[n] + m_1 t + A \, \text{sin}(\omega  t+\varphi) \right) u(t) {\ast} h(t)\bigg\rvert_{t=t_{\text{on}}[n]}.
% \end{align}
We observe that in constant on(off)-time control, $\psi_2$ is a pure gain, however, in fixed-frequency control, the $\psi_2$ introduces a pole at $z=0$ and a zero. The simplified root locus of the current-control loop is shown in Fig.\;\ref{fig:fpcc_filter}. 
\begin{figure}
    \centering
    \includegraphics[width = 8cm]{filter_fpcc.pdf}
    \caption{Root locus for fixed-frequency current-control block without (left)/with (right) filter: %\multiput(0,0)(3,6){5}{\line(1,2){2}}
    {\color{green}---} is for the negative feedback; {\color{blue} -\,-\,-} is for the positive feedback.}
    \label{fig:fpcc_filter}
\end{figure}
% We observe that the location of pole $a^i_1$ is dependent on the phase $\phi$ and frequency $\omega$ of the interference function $f$. To guarantee the stability within all phases $\phi$ and frequency $\omega$, 

% \begin{align}
%      k(\tau, \omega) =  \left( \frac{ \frac{1}{\omega^2 \tau}}{\left(1-e^{-(T_\text{on}+T_{\text{off}})/\tau}\right)}\right) \frac{e^{-(T_{\text{on}} +T_{\text{off}}) /\tau}}{\tau m_1} + \frac{ 1}{\omega \tau }\\
%      l(\tau) =  \left( \frac{(T_{\text{on}}+\tau e^{-T_{\text{on}}/\tau}-\tau)}{\left(1-e^{-(T_\text{on}+T_{\text{off}})/\tau}\right)}\right) \frac{e^{-(T_{\text{on}} +T_{\text{off}}) /\tau}}{\tau m_1}
% \end{align}
% For the ease of calculation, we denote
% \begin{align}
%     p(\tau) = \left( \frac{ 1}{\left(1-e^{-(T_\text{on}+T_{\text{off}})/\tau}\right)}\right) \frac{e^{-(T_{\text{on}} +T_{\text{off}}) /\tau}}{ m_1}
% \end{align}
% Then the $k_1$ can be expressed as：
% \begin{align}
%     k(\tau, \omega) = \frac{p(\tau)}{(\omega \tau)^2} + \frac{1}{\omega \tau} 
% \end{align}
% From the theorem x, we have the stability condition is
% \begin{align}
%     (k \frac{A \omega}{m_1} +l) & < \frac{1}{2} \nonumber \\
%     (\frac{p(\tau)}{(\omega \tau)^2} + \frac{1}{\omega \tau}) \frac{A\omega}{m_1} + l(\tau) &< \frac{1}{2}
% \end{align}
% From the theorem x, we have the stability condition is. Therefore, to guarantee the stability of inner current loop, the filter $\tau$ has to satisfy
% \begin{align}
%     \left(\frac{p(\tau)}{(\omega_{\text{min}} \tau)^2} + \frac{1}{\omega_{\text{min}} \tau} \right) \frac{A_{\text{max}} \omega_{\text{min}}}{m_1} + l(\tau) - \frac{1}{2} < 0
% \end{align}

% For any operating point, the $a^i_1$ is within the range 
% \begin{align}
%     a^i_{1_{\text{l}}} &=  1 - \frac{1}{1-\frac{A}{m_1(\tau+1/2\pi f) \gamma} + \frac{a}{\gamma}} \le a^i_1 \nonumber \\
%  &\le a^i_{1_{\text{u}}} = 1- \frac{1}{1 + \frac{A}{m_1(\tau+1/2\pi f)\gamma}+ \frac{a}{\gamma}}
% \end{align}

% \begin{align} \label{SC31}
% a^i_{1_{\text{l}}} &=  1 - \frac{1}{1-e^{-\frac{T_{\text{on}}}{\tau}}-\frac{A}{m_1(\tau+1/2\pi f)}} \le a^i_1 \nonumber \\
% &\le a^i_{1_{\text{u}}} = 1 - \frac{\gamma}{1-e^{-\frac{T_{\text{on}}}{\tau}} + \frac{A}{m_1(\tau+1/2\pi f)}}
% \end{align}
% We can prove $|a^i_{1_{\text{l}}}|>|a^i_{1_{\text{u}}}|$ from (\ref{SC31}) and mean inequality,
% \begin{align} \label{SC32}
% 1 < \frac{2}{\frac{1}{1-a^i_{1_{\text{l}}}}+\frac{1}{1-a^i_{1_{\text{u}}}}} \le \frac{(1-a^i_{1_{\text{l}}}) + (1 -a^i_{1_{\text{u}} })}{2}
% \end{align}
% Therefore the worst-case pole locates at $a^i_{1_{\text{l}}}$. We want to maximize the $a^i_{1_{\text{l}}}$. 
% We simplify $a^i_{1_{\text{l}}}$ as 
% \begin{align} \label{SC31}
% a^i_{1_{\text{l}}} &=  1 - \frac{1}{1-e^{-\frac{T_{\text{on}}}{\tau}}-\frac{A}{m_1\tau}} 
% \end{align}
% Denote $\tau_i = 1/\tau$, 
% \begin{align} \label{SC31}
% a^i_{1_{\text{l}}} &=  1 - \frac{1}{1-e^{-T_{\text{on}} \tau_i}-\frac{A}{m_1}\tau_i} 
% \end{align}
% From zero gradient condition, we know at $\hat{\tau} = \frac{\ln(\frac{m_1T_{\text{on}}}{A})}{T_{\text{on}}}$, 
% \begin{align}
% a^i_{1_w} = 1 - \frac{1}{1-e^{-\frac{T_{\text{on}}}{\hat{\tau}}}-\frac{A}{m_1\hat{\tau}}}
% \end{align}
% $a^i_{1_w} $ is where the optimal worst-case pole is.




% \begin{table}
%     \caption{Parameters that prove nothing is impossible. This life is nothing short of an awakening spark of heroic healing.}
%     \label{table:curr_rect_params}
%     \centering
%     \begin{tabular}{ccccccccc}
%         \toprule
%         $P_o$&$Q_o$&$ r $&$H_1$, $H_2$&$U_{extra}$&$B_{L}$&$B_o$, $K_b$&$M$&$Y_s$    \\
%         \text{[mm]}&[cm]&[hPa]&Ion Number&[Energy]&[Universe]&[QQQ]&[AK]&[AQ]    \\
%         \midrule
%         500&100&27.12&\textit{ABCDEFG}&26&5&6&498&333 \\
%         \bottomrule
%     \end{tabular}
%     \vspace{-10pt}
% \end{table}

% \subsubsection{Highlight}
We show a rigorous analytic way to design filter. In \mbox{traditional} way of designing filter, LPF are commonly designed to cut off after the switching frequency and far before the interference. This makes the filters cannot effectively suppress the interference whose spectrum is around or below the switching frequency. In our way of designing filter, we select the filter time constant by accurate design equation. The cut-off frequency of filter is allowed to be well-below the switching frequency and still result in good performance. Even the bandwidth of the filter is so low that ramp is distorted, the performance of the current-control loop is still acceptable.
LPF has a symmetric effect on the peak current-mode control and valley current-mode control. A low pass filter with low cut off frequency compared to switching frequency has a severe stabilizing effect on the valley current-mode control.


==> 4_solution_sc.tex <==
\subsection{Slope Compensation} \label{sec:solution_subsec:slopecompensation}
Slope compensation is a well-recognized control conditioning method that stabilizes the fixed-frequency current-mode control loop when the duty cycle crosses 50\,\%.
What had been previously unknown is that slope compensation can also be used for the control conditioning of interference.
% We explore the new applications of slope compensation for interference conditioning in both constant on-time and fixed-frequency current-mode controller.
Slope compensation can repair both discontinuities and the ensuing smooth nonlinearities in the static mapping, as well as improving the transient performance of the dynamical mapping.
Slope compensation decreases the degree of nonlinearity by effectively flattening the interference in the time domain waveform as shown in Fig.\,\ref{fig:slope_w_inf_td}. This has the consequence of flattening the static mapping by contracting the points in the interference that correspond to early triggering (negative deviation from transformed ideal line of the current mapping) and late triggering (positive deviation from the transformed ideal line) as illustrated in Fig.\,\ref{fig:slope_w_inf_td}.  For an ideal static mapping, slope compensation does not introduce nonlinearities, but rather introduces a slope (gain) error in the mapping, as shown in Fig.\,\ref{fig:slope_no_inf}.  As previously mentioned, this gain error is outside of the current control loop and is subsequently corrected in the design of the outer voltage loop.
\begin{figure}
    \centering
    \includegraphics[width = 8cm]{slope_w_inf_td.pdf}
    \caption{Time domain explanation of how slope compensation conditions the interference. Slope compensation guarantees the continuity of the static current mapping by rotating the current sensor signal until it becomes monotonic and re-scaling the deviation from the interference.}
    \label{fig:slope_w_inf_td}
\end{figure}
% The extra negative slope is equivalently an extra positive slope on the current ramp. It improves the signal-to-interference ratio of the sensed inductor current by enhancing the signal as shown in Fig.\;\ref{fig:sc1}. Hence the stability of current-controller is improved.
% \begin{figure}
%     \centering
%     \includegraphics[width=8cm]{slopecomp.pdf}
%     \caption{ \label{fig:sc1} Comparison of the current-sense voltage with/without slope compensation. {\color{blue}---} is for the current-sense voltage without slope compensation. {\color{orange}$\cdots$} is for the current-sense voltage with slope compensation. {\color{red}-\,-\,-} is for the compensation slope.}
% \end{figure}
\begin{figure}
    \centering
    \includegraphics[width = 6cm]{slope_w_inf.pdf}
    \caption{Slope compensation weakens the nonlinearity of the static current mapping by contracting the deviation from the ideal triggering.}
    \label{fig:slope_w_inf}
\end{figure}
\begin{figure}
    \centering
    \includegraphics{slope_no_inf.pdf}
    \caption{Slope compensation does not affect the nonlinearity of the static current mapping but causes a gain error on the mapping.}
    \label{fig:slope_no_inf}
\end{figure}

% \subsubsection{Modeling of the current-controller with Slope Compensation}
We start with constant off-time current-mode control as an example.
By adding slope compensation, we replace $i_c$, which is constant within every switching cycle, with \mbox{$i_c - m_s t$}, which is a decreasing ramp for $m_s>0$.
A state-space form of the current control loop is
\begin{subequations}
\label{eqn:slopecompsys}
    \begin{align}
     \label{eqn:slopecompsysip} i_p[n] &= i_p[n-1] - m_2T_{\text{off}} +m_1t_{\text{on}}[n], \\
     \label{eqn:slopecompsysic} i_c [n]  &= i_p[n] + w(t_{\text{on}}[n]) + m_s t_{\text{on}}[n].
    \end{align}
\end{subequations}

%\begin{subequations}
%\label{eq:Maxwell}
%Maxwell's equations:
%\begin{align}
%        B'&=-\nabla \times E,         \label{eq:MaxB} \\
%        E'&=\nabla \times B - 4\pi j, \label{eq:MaxE}
%\end{align}
%\end{subequations}

% \subsubsection{Stability Analysis}
% The Proposition\,\ref{th:equexcond} indicates that the static current mapping is continuous if and only if the inference does not affect the monotonicity of the current sensor output.

Proposition\,\ref{th:equexcond} in Section\,\ref{sec:fet_latching} states that if the current sensor output is not monotonic, then the static current mapping is discontinuous. A discontinuous static mapping can make the current control loop unstable. 
Corollary\,\ref{reachthoerem:slopecomp_constontime} below states that if a slope compensation $m_s$ is added, the discontinuity can be eliminated as had been discussed for Fig.\,\ref{fig:slope_w_inf_td}.
We show that an appropriately designed slope compensation can make the time-domain function of the current sensor output monotonic; by Proposition\,\ref{th:equexcond}, the static mapping is also made continuous.
\begin{corollary} \label{reachthoerem:slopecomp_constontime}
$\mathcal{T}$ is a strictly monotonically increasing and continuous static mapping if and only if  \mbox{$(m_1 + m_s)\,t+w(t)$} is strictly monotonically increasing and continuous within a switching cycle.
\end{corollary}
The proof relies on the similarity of system
(\ref{eqn:slopecompsys}) with (\ref{eqn:cmcotshiftlin}), hence it is omitted in this paper.

In this section, we show that adding an extra slope transforms both the interference and the ideal current ramp, which allows the dynamical mapping to be stabilized even if the original interference violates the stability bound in Theorem\,\ref{theorem:gloasystab}. From Theorem \ref{theorem:gloasystab} and having satisfied its condition of continuous static mapping, the stability of the dynamical mapping depends on the upper bound of the Lipschitz constant $\Lambda_{ub}$ of the interference.  For a larger $\Lambda_{ub}$, an accordingly larger $m_s$ is needed to make the current control loop globally asymptotically stable.

This slope compensation method does not impose any restrictions on the amplitude and frequency of the interference, which means it can be an often-used and robust large-signal method to stabilize the current control loop.  One proviso is that a larger compensation $m_s$ corresponds to a higher loop gain, hence moving the pole on the $z$-domain root locus as we explain below; when it is too high, it slows down the closed\nobreakdash-loop response of the current control loop, which is the opposite of what happens in the $s$-domain when the loop gain becomes higher.

%{\color{red} For the same amplitude, higher frequency interference %= higher Lipschitz constant.
%So need higher slope compensation.
%Higher slope compensation means higher loop gain, which moves the %pole from the origin towards the unit circle -->  slowing down the %loop bandwidth.
%}

We approach the stability analysis by applying the $z$\nobreakdash-transform to system (\ref{eqn:slopecompsys}).
The current control loop can be represented as the Lure system in Fig.\;\ref{fig:sccotcmblockdiagram}.
$G(z)$ can be found in (\ref{eqn:gzofcotcm}). %(\ref{eqn:cmcotip_sc}) and %(\ref{eqn:cmcotic_sc}) 
% \begin{align}
%     G(z) = \frac{1-z^{-1}}{m_1}.
% \end{align}
The interference is embedded in the static nonlinearity $\psi_1$ in the feedback path
\begin{align}
    \psi_1 = w(\tilde{t}_{\text{on}}[n]).
\end{align}
The slope compensation is embedded as a gain $\psi_2$ also in the feedback path 
\begin{align}
    \psi_2 = m_s.
\end{align}
% \begin{align} \label{eqn:S2_2}
% s = \frac{f^{'}(T_{\text{on}}) + m_s}{m_1}.
% \end{align}
If the function $w(\cdot)$ is monotonically decreasing, 
the feedback path $\psi_1$ is a positive feedback path and might cause instability.
Typically the compensation slope $m_s$ is chosen to be positive, which makes $\psi_2$ a negative feedback path, which can be used to correct the destabilizing effect of $\psi_1$.

As a Lure system, we can apply the circle criterion, which is illustrated in Fig.\,\ref{fig:slope_no_inf}; the large-signal stability criterion for the dynamical mapping can be proven.
\begin{corollary} \label{stabthoerem:slopecomp_constontime}
The current control loop represented by the Lure system in Fig.\,\ref{fig:sccotcmblockdiagram} is \emph{globally asymptotically stable} if \mbox{${\Lambda}_{ub} < m_1/2 + m_s$}.
\end{corollary}
The proof is similar to  Theorem\,\ref{theorem:gloasystab}, hence omitted in this paper.
% \begin{figure}
% ~
% \begin{minipage}{0.5\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{sc_cotcm.pdf}
%   \caption{\label{fig:sc2} Root locus of the current-controller of constant on(off)-time control without(left)/with(right) the slope compensation. The solid green line is for the negative feedback and the dotted blue line is for the negative feedback.}
% \end{minipage}
% % ~
% % \begin{minipage}{0.32\textwidth}
% %     \centering
% %     \includegraphics[width=\textwidth]{Figure/section3/copd/physicalmodelcomp.PNG}
% %     \caption{\label{fig:physicalmodel} Simplified physical model of a comparator.}
% % \end{minipage}
% \end{figure}

% we start the subfig here
\begin{figure}
    \centering
    \includegraphics[width=6cm]{blockdiagramsc.pdf}
    \caption{Block diagram of the constant off-time/fixed-frequency peak current control loop with the slope compensation. The interference is embedded in $\psi_1$ and the slope compensation is embedded in $\psi_2$.}
    \label{fig:sccotcmblockdiagram}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=5 cm]{sc_cotcm_new.pdf}
    \caption{Small-signal root locus of the constant off(on)-time current control loop with the slope compensation. The sign of the feedback is determined by the interference.  In positive feedback, slope compensation decreases the loop gain to increase the stability margin.  In negative feedback, the converter is always stable, but results in a slower transient performance. In practice, the polarity of the feedback cannot be determined a-priori and the compensation slope is chosen so that the converter is stable in positive feedback.}
    \label{fig:sc_cotcm_new}
\end{figure}
We can obtain an intuition for stability by examining the linearized system for (\ref{eqn:slopecompsys}).
% \begin{align} 
% \label{eqn:cmcotip_sc} \tilde i_p[n] &= \tilde i_p[n-1] +  m_1 \tilde t_{\text{on}}[n], \\
% \label{eqn:cmcotic_sc} \tilde i_c [n]  & = \tilde i_p[n] + (f^{'}(T_{\text{on}}) +m_s)\tilde t_{\text{on}} [n].
% \end{align}
% We normalize the slope by defining the slope ratio $\gamma = m_s/m_1$ and $s = f^{'}(T_{\text{on}})/m_1$. 
The root locus for this linearized system is illustrated in Fig.\,\ref{fig:sc_cotcm_new} and helps to visualize how slope compensation improves stability and affects the transient response. 
% The slope compensation right shifts the poles which were outside of the unit-cycle into the unit-cycle.
% Slope compensation can make unstable poles into stable poles; it does this by right shifting the poles into the unit circle.
% Performance analysis, by doing linearization and Z-transform
% The small-signal model is:
% \begin{align}
% \tilde i_p[n] &= \tilde i_p[n-1] +  m_1 \tilde t_{\text{on}}[n], \\
% \tilde i_c [n] - m_s \tilde t_{\text{on}} [n] & = \tilde i_p[n] + f(t_{\text{on}}[n]) - f(T_{\text{on}}).
% \end{align}
% Then the new nonlinear static function is $\psi(y) = m_1 \phi ^{-1}(y-f(T_{\text{on}}))$, where $\phi(x) = m_s x + f(x)$. If (\ref{sc1}) holds, we can confidently say the oscillation cannot sustain in the inner loop. 
% \begin{align} \label{sc1}
% m_s + (f')_{\text{min}} > -m_1/2
% \end{align}
% \subsubsection{Transient Performance Analysis}
% {\color{red} (revised by XC for review) If the interference causes a positive feedback path, the closed-loop pole locates at the left half plane and may be outside of the unit circle as shown in Fig.\,\ref{fig:sc2}(a).
% Adding the slope compensation can right shift the unstable pole into the unit cycle so that the current control loop is stabilized as shown in Fig,\,(b).
% If the interference causes a negative feedback path, the closed-loop pole locates at the right half plane as shown in Fig.\,\ref{fig:sc2}(c).
% Adding the slope compensation may right shift the closed-loop pole towards $z = 1$ and increase the worst-case settling.
% }
We observe that slope compensation for positive feedback in Figs.\,\ref{fig:sc_cotcm_new} (a) and (b) moves the location of the worst\nobreakdash-case closed-loop pole further to the right, hence improving stability margin.  Likewise, for negative feedback in Figs.\,\ref{fig:sc_cotcm_new} (c) and (d), adding the slope compensation right\nobreakdash-translates the closed\nobreakdash-loop pole towards \mbox{$z = 1$} and increases the worst-case settling.
% So there exists a $\tau_{\text{min}}$ such that for all $\tau > \tau_{\text{min}}$, all the poles of the current-command block can stay inside the unit-cycle. The following Theorem provides an accurate design method for the filter.

We use the settling and overshoot metrics in (\ref{eqn:settlecycle1}) and (\ref{eqn:overshoot1}), respectively, to quantitatively illustrate the relationship between these metrics and the pole locations. With interference, the pole $a$ cannot be located exactly, but rather within a range $[a_{\text{min}},a_{\text{max}}]$, where
\begin{align} %\label{eqn:range_pole_sc}
a_{\text{min}} = \frac{m_s-{\Lambda}_{ub}}{(m_1 + m_s - {\Lambda}_{ub})},  
\,a_{\text{max}} = \frac{m_s+{\Lambda}_{ub}}{(m_1 + m_s + {\Lambda}_{ub})}.
\end{align}
The worst-case for settling and overshoot can be obtained from (\ref{eqn:settlecycle1}) and (\ref{eqn:overshoot1}), respectively.  It is worth noting that $a_{\text{min}}$ and $a_{\text{max}}$ are not usually symmetric about the origin.

The transient performance of the current control loop varies with the compensation slope, as shown in Fig.\,\ref{fig:scsettlingtime} and Fig.\,\ref{fig:scovershoot}.
The transient performance is related to the \emph{normalized} compensation slope $\hat{m}_s$ and \emph{normalized} Lipschitz constant of interference $\hat{\Lambda}_{ub}$
\begin{align} \label{eqn:ms_norm}
    \hat{m}_s \triangleq \frac{m_s}{m_1},\quad \quad \hat{\Lambda}_{ub} \triangleq \frac{{\Lambda}_{ub}}{m_1}.
\end{align}

The curves from Fig.\,\ref{fig:scsettlingtime} are convex with points of minimum settling, which are marked by symbol points on each of the curves. The worst-case overshoot decreases monotonically with the compensation slope as shown in Fig.\,\ref{fig:scovershoot}. These show a tradeoff between settling and overshoot.
\begin{figure}[ht]
\centering
\subfigure[The worst-case settling $N_w$ decreases first and then increases with the compensation slope $\hat{m}_s$.]{
\includegraphics[width=6 cm]{settlingtime_final.pdf} \label{fig:scsettlingtime}
}
\subfigure[The worst-case overshoot $O_w$ decreases with the compensation slope $\hat{m}_s$.]{
    \includegraphics[width=6 cm]{overshoot_final.pdf}  \label{fig:scovershoot}
}
\caption{The control conditioning diagram for compensation slopes given different interference levels $\hat{\Lambda}_{ub}$ \red{change this $L$ to be $\Lambda$}. For a given interference, there is a minimum settling $N_w$ required. Beyond a certain compensation slope, the overshoot is always zero, but the penalty in $N_w$ keeps increasing.}
% Caption for if you have a tradeoff curve:  For a given interference, there is a minimum settling $N_w$ required and beyond a certain compensation slope, the overshoot is always zero, but the penalty in $N_w$ keeps increasing; this is exemplified in the tradeoff curve.
%\label{fig:subfigureExample}
\end{figure}
%Therefore, given any design objective which can be formulated as a combination of settling time and overshoot, the optimal slope can be found by the control conditioning diagram. 
The range of pole locations can be expressed as
\begin{align} %\label{eqn:range_pole_sc}
a_{\text{min}} = \frac{\hat{m}_s-\hat{\Lambda}_{ub}}{(1 + \hat{m}_s - \hat{\Lambda}_{ub})}, a_{\text{max}} & = \frac{\hat{m}_s + \hat{\Lambda}_{ub}}{(1 + \hat{m}_s + \hat{\Lambda}_{ub})}.
\end{align}
% The compensation $\hat{m}_s$ over different degrees of interference $\hat{\Lambda}_{ub}$ are shown in Fig.\,\ref{fig:scsettlingtime}.
By observing that the bounds $a_{\text{min}}$ and  $a_{\text{max}}$ monotonically move to the right in the root locus with increasing $\hat{m}_s$, the criterion for minimum worst-case settling is then $a_{\text{min}} = -a_{\text{max}}$, from which the corresponding $\hat{m}_s^*$ can be solved
\begin{align} \label{eqn:optms}
     \hat{m}_s^* & = \sqrt{\frac{1}{4} + {\hat{\Lambda}_{ub}}^2} - \frac{1}{2}.
\end{align}
% The detailed proof can be found in Appendix  \ref{sec:proofoptsc}.
The corresponding minimum worst-case settling is
\begin{align} \label{eqn:th_wc_settling}
    N_w^* = 
    \Bigg|\frac{4}{\text{ln}\Big|1 - (1 + \sqrt{\frac{1}{4}+{\hat{\Lambda}_{ub}}^2} + \hat{\Lambda}_{ub})^{-1}\Big|}\Bigg|.
\end{align}


% The effect of poles by the ramp compensation
% Formulate an optimization

% \subsubsection{Analysis on Constant On-time and Fixed-frequency current-controller}
These results can be extended to other types of current control loops.
The continuity theorem, stability theorem, and the performance analysis for constant on-time control can be derived by exchanging $m_1$ and $m_2$ in $G(z)$.
The result for fixed-frequency control can be derived by substituting ($\ref{eqn:fpccplanttf}$) for $G(z)$.  The effect of slope \mbox{compensation} on the root locus for fixed-frequency control is shown in Fig.\;\ref{fig:rl_fpcc_sc}.
\begin{figure}
    \centering
    \includegraphics[width = 5cm]{sc_fpcc.pdf}
    \caption{Small-signal root locus for fixed-frequency current control loop with the slope compensation.
    The sign of the feedback is determined by the interference.  In positive feedback, slope compensation decreases the loop gain to increase the stability margin.  In negative feedback, the converter is always stable, but results in a slower transient performance. In practice, the polarity of the feedback cannot be determined a-priori and the compensation slope is chosen so that the converter is stable in positive feedback.}
    \label{fig:rl_fpcc_sc}
\end{figure}
% \subsubsection{Highlights} 

% The design guide includes ensuring global asymptotic stability, choosing a feasible settling and \mbox{overshoot} through the tradeoff curve, and finding the optimal \mbox{compensation} slope.

==> 5_5_HardwareDemo.tex <==
\section{Hardware Results} \label{sec:hardwaredesignguide}
% {\red{UNEMBEDDED IT The design of a controller for a current-mode converter 
% includes both the current-control and voltage-control loops.
% % The voltage-control loop design is omitted in this paper and will be discussed in the future paper.
% current control loop design requires three steps: (i) selecting the current-control mode of operation;\footnote{Fixed-frequency peak/valley or variable-frequency constant-on/off time.} (ii) characterizing the interference; and (iii) choosing and designing the control conditioning.
% The overall design procedure is summarized in Fig.\,\ref{fig:designflow_cmc}.}}

In this section, 
%we use the hardware results to demonstrate the effectiveness of slope compensation as control conditioning.
% The design guide uses the analytical results developed in Sections\,\ref{sec:modeling} and \,\ref{sec:solution}. 
% We first apply the appropriate stability criterion to obtain the feasible range of design parameters.
% Within this feasible range, we then design for transient performance, which include the overshoot and settling.
a multi-megahertz buck converter prototype \cite{Cui2018a} is used as a working hardware example to demonstrate the effectiveness of control conditioning for current control loops with interference dysfunction.
For this prototype, we selected constant on-time current-mode control, which is frequently used in high-speed converters for microprocessors \cite{Wong1998}.
\subsection{Hardware Prototype}
The conditioning method in this paper applies for conditioning the effects of interference that occurs in all types of current sensors. 
We use the ground-referenced shunt\nobreakdash-resistor current sensor as an example because of its simplicity and wide measurement bandwidth.
The parameters for the constant on\nobreakdash-time buck converter can be found in Table\;\ref{table:cotcm_buck_param}.
\begin{table}[tb]
    \caption{Design Parameters of the Constant On-Time Current-Mode Buck Converter}
    \label{table:cotcm_buck_param}
    \centering
    \begin{tabular}{cccccccccccccc}
        \toprule
\textbf{Parameters}&\textbf{Values}&\textbf{Parameters}&\textbf{Values}\\
\midrule
$\mathbf{V_{\textbf{in}}}$
& 12\,V & $\mathbf{L}$ & 240\,nH\\
\midrule
$\mathbf{V_{\textbf{out}}}$
& 2\,V & $\mathbf{R_{\textbf{sample}}}$
& 10\,m$\Omega$ \\
\midrule
$\mathbf{I_{\textbf{out}}}$ 
& 8\,A & $\mathbf{f_{\textbf{int}}}$
& 5\,MHz \\
\midrule
$\mathbf{T_{\textbf{on}}}$ 
& 100\,ns & $\mathbf{A_{\textbf{int}}}$
& 4\,mV \\
\midrule
$\mathbf{C}$ & 100 $\mu$F &
& \\
%$\mathbf{T^{\textbf{min}}_{\textbf{off}}}$  & 175\,ns \\
        \bottomrule
    \end{tabular}
\end{table}
A  %control algorithm is implemented %digitally and 
photograph of the prototype is shown in Fig.\,\ref{fig:exp_ebuck_2}.
\begin{figure}[ht]
        \centering
        \includegraphics[width = 6 cm]{exp_ebuck_2.pdf}
        \caption{A 30W, 5 MHz current-mode buck converter using constant on-time cycle-by-cycle digital control \cite{Cui2018a}. The digital controller is implemented in a Xilinx Artix-7 FPGA, which makes the controller flexible, adaptable, and re-programmable.
        % A 30\,W, 5\,MHz current-mode buck converter using constant on-time under test. The digital control is implemented in FPGA.
        }
        \label{fig:exp_ebuck_2}
\end{figure}
\begin{comment}
\subsection{Comparisons of Three Interference Conditioning Methods}
\label{sec:performancecomp}
\begin{figure*}
    \centering
    \includegraphics[width=18cm]{section3/general/designflow_cmc.pdf}
    \caption{Design procedure of current mode control include two steps as shown in the top blue layer. Current controller design include three steps as shown in the middle red layer. Current conditioning design include three steps as shown in the bottom green layer. }
    \label{fig:designflow_cmc}
\end{figure*}
Slope compensation, low-pass filtering, and comparator-overdrive-delay conditioning can each be independently used to repair defective static and dynamic mappings that are caused by interference. 
% We would like to compare the pros and Cons on different methods.
We show a unified framework for comparing the three control conditioning methods.  All three methods can decrease the degree of nonlinearity in the static mapping, but introduce other non-idealities that must be accounted.  Low-pass filtering repairs the original nonlinearity, but introduces a different nonlinearity in the current sensor output; these two nonlinearities must be balanced to minimize the overall nonlinearity.
Slope compensation adds a gain error and 
comparator-overdrive-delay conditioning causes an offset error in the static mappings.

All three methods can improve the stability margin and transient response of current control loops with interference dysfunction.
To compare control-conditioning methods, we choose overshoot as a metric for stability margin and settling as a metric for transient response.
\begin{figure}[ht]
\centering
\subfigure[Normalized amplitude $\hat{A} = 0.01$, Normalized frequency $\hat{\omega} = 3$ ({\color{red} in the picture change the $A^*$ to $\hat{A}$ and change the $\omega^*$ to $\hat{\omega}$ }.
)]{
\includegraphics[width=8 cm]{comparision_A_001_w_3.pdf}\label{fig:comparision_a_001_w3}
}
\newline
\subfigure[Normalized amplitude $\hat{A} = 0.12$, Normalized frequency $\hat{\omega} = 1$]{
    \includegraphics[width=8 cm]{comparision_A_012_w_1.pdf} 
    \label{fig:comparision_a_012_w1}
}
\caption{Overshoot-settling cycle performance tradeoff. Three interference conditioning methods are compared on a current-mode converter using constant on/off-time control. The $\hat{A}$ and $\hat{\omega}$, which will be defined in Section \ref{subsection:opddesignguide}, are the normalized amplitude and frequency of interference.
The $\tau^*$, which will be defined in Section \ref{subsection:lpf}, is the normalized time constant of filter.}
%\label{fig:subfigureExample}
\end{figure}

It is incomplete to compare either the settling or overshoot alone because each method has \emph{design parameters} which allow designers to trade-off between these two performance metrics, hence we construct a two-dimensional performance space as shown in Figs.\,\ref{fig:comparision_a_001_w3} and \ref{fig:comparision_a_012_w1}. By sweeping the key design parameter for each method, i.e. comparator time constant, compensation slope, and filter time constant, we can plot the point set for the three methods in this space; points closer to the origin have a better performance tradeoff in overshoot and settling. These curves depend on the interference parameters $(\hat{A}, \hat{\omega})$, with all methods performing worse with higher interference amplitude. 

Fig. \ref{fig:comparision_a_001_w3} illustrates that if the interference frequency is far enough above the switching frequency (e.g. $\omega = 3\,\omega_{sw}$), both the comparator-overdrive-delay conditioning and low-pass filter can achieve a smaller overshoot and shorter settling than slope compensation.
Fig. \ref{fig:comparision_a_012_w1} illustrates that if the interference frequency is comparable to the switching frequency (e.g. $\omega = 3\,\omega_{sw}$), comparator overdrive-delay-conditioning and slope compensation can result in a smaller overshoot and shorter settling than the low-pass filter.
\begin{table*}[tb]
    \caption{Comparison of Three Conditioning Methods}
    \label{table:cond_compare}
    \centering
    \begin{tabular}{cccccccccccccc}
  \toprule
\textbf{Method}
&\textbf{Less} &\textbf{Large-Signal}
&\textbf{Transient Performance}
&\textbf{Transient Performance}
\\
\textbf{}
&\textbf{Complexity} &\textbf{Design Performance}
&\textbf{@ $\omega \gg \omega_{\text{int}}$}
&\textbf{@ $\omega \approx \omega_{\text{int}}$}
\\
\midrule
\textbf{Filter}
& +++ & + & ++ &  + \\
\midrule
\textbf{Slope Compensation} 
& ++ & +++ & + & ++ & \\
\midrule
\textbf{Comparator Overdrive}  
& + & ++
& +++ & +++ \\
%$\mathbf{T^{\textbf{min}}_{\textbf{off}}}$  & 175\,ns \\
        \bottomrule
    \end{tabular}
\end{table*}

The comparison of three conditioning methods is summarized in Table\,\ref{table:cond_compare}.
``Large Signal Design Performance'' describes how the large signal stability criterion affects the small-signal transient performance, which indicates the large-signal transient performance.
For example, as shown in Fig.\,\ref{fig:opdr_settlingtime}, when the large-signal design performance gets worse, the tradeoff curve between the comparator time constant and settling moves away from the origin.
Filter is advantageous in low implementation complexity. However, the large-signal criterion of the filter is most conservative out of all methods, therefore it results more stringent performance penalties.
Slope compensation provides the least-conservative large-signal stability criterion among the three methods. But the transient performance largely degrades if the interference frequency is much higher than the switching frequency. 
Comparator overdrive exhibits the best small-signal performance for the interference that is comparable or faster than switching frequency. However, there only exists a limited set of commercially available comparators. So the design is likely to be far from optimal. A customized integrated circuit allows the continuous tuning of overdrive, whereas, the cost of implementation is high.

We show an intuitive explanation on why the comparator overdrive can outperform the rest of two methods. The comparator overdrive attenuates the interference without influencing the original current ramp. In contrast, the slope compensation adds an extra ramp on the original ramp. The filter cannot avoid distorting the original ramp when filtering the interference. Besides, it is easier to implement the comparator overdrive in the integrated circuit because the comparator gain can be well-controlled by online programming the tail current.
\end{comment}

%\subsection{Interference Characterization}
% The first step is to select a mode of operation. The operation modes may include fixed-frequency peak/valley current-mode control, constant-on/off time current-mode control and etc.
% We select the constant on-time current-mode control because this type of converter is widely used in powering the digital integrated circuit for computation.

% We need to extract the interference parameter from experimental waveform.
\begin{figure}[ht]
\centering
    \subfigure[Current sensor output of the buck converter running at 1\,MHz in steady state.]{
    \centering
    \includegraphics[width= 6 cm]{Intf1mhz.PNG}
    \label{fig:Intf1mhz}
    }
    \subfigure[Current sensor output of the buck converter running at 2\,MHz in steady state.]{
    \centering
    \includegraphics[width = 6 cm]{Intf2mhz.PNG}
    \label{fig:Intf2mhz}
    }
    \caption{Interference in the power converters is near the switching frequency. Channel 1 (dark blue) represents the voltage between the current-sense resistor and comparator ground. Channel 2 (light blue) represents the voltage cross the converter ground and comparator ground. Channel M indicates the voltage difference Channel 2 minus Channel 1. Channel 3 (pink) shows the inductor current.}
\end{figure}
\begin{figure}
    \centering
    \includegraphics{sch_ebuck.pdf}
    \caption{Current-mode buck converter using constant on-time.}
    \label{fig:sch_buck}
\end{figure}
A ground-referenced, current-sense resistor is placed on the source of the low-side switch of the buck converter prototype as shown in Fig.\,\ref{fig:sch_buck}.
The inductor current rises when the high-side switch is on and falls when the high-side switch is off as illustrated in Fig.\,\ref{fig:subharmonicscurrent}. 
The current sensor voltage is negative and trapezoidal.  The actual current sensor waveforms in Fig.\,\ref{fig:subharmonicscurrent} contain a significant amount of interference that is problematic at multi\nobreakdash-MHz switching frequencies.

% The first step is to classify the interference. There are two basic classifications: (i) a {\em simple interference} is dominated by a decaying single-frequency sine wave; and (ii) a {\em complex interference} which is a complicated waveform and hence consists of multiple frequency components.

% In this example, we observe there is mainly one under-damped oscillation mode, hence we use its sinusoidal envelope as a conservative estimation. The amplitude and frequency is shown in Table\,\ref{table:cotcm_buck_param}.
% If I am willing to do frequency decomposition, but want $A_{ub}$ to be independent from $f_c$, 
% For the current sensor waveform that is more complicated, for example, containing more than one frequency component,  
% We provide the following method which systematically bounds on the magnitude spectrum of interference.
% We subtract the ramp, get pure $w(t)$, do short time Fourier Transform to get the spectrum.
% If interference is periodic for multi period, we
% We record the long-enough current sensor waveform so that at least one period of the interference is included. 
% We then substract the ideal trapezoidal waveform from the current sensor waveform to get the pure interference signal.
% We apply the Fourier Transform to the resulting signal and get the magnitude spectrum of interference.
% The upper bound of the amplitude of interference $A_{ub}$ can be estimated by adding up all Fourier coefficients as shown in (\ref{eqn:aub}).
% However, depending on the magnitude spectrum, the $A_{ub}$ may be too conservative and causes the subsequent control conditioning design infeasible or over conservative.

% In case that $A_{ub}$ in the above is infeasible or too conservative, we show three categorical interference class which can possibly allow us to have a tighter design by having a better estimation of $A_{ub}$ .
% 1)\,If the class of interference is dominated by the low frequency in energy, we can put a
% low-pass signal filter nearby the low frequency component but much higher than the switching frequency. Hence we can estimate the $A_{ub}$ by ignoring the other high frequency components.
% 2)\,If the class of interference has both low frequency and high frequency components with high energy, we may use the iterative design to decide the cut-off frequency of the signal filter. 
% The heuristic starting point can be set nearby the low frequency component.
% However, it is worth noticing that if there are high-frequency ringings with high energy, the current sensor circuit may not behavior well.
% 3)\,if the class of interference is undetermined, we might need to directly solve the optimal cut-off frequency problem of the signal filter. 
% It is a non-convex optimization problem and result in a locally optimal cut-off frequency for the signal filter design.

% For comparator overdrive, $A_{ub}$ can be a largest signal amplitude in region B,C and D.

% {\color{blue}For Figs 38, in this framework, we only care about small signal performance, Hence both the overshoot and settling of the comparator is better as the comparator is getting slower 
% showing the arrows for legend 
% and how omega varies
% cricle the optimal/tradeoff cruve
% There is no tradeoff between the overshoot and settling
% There is only one optimal point for the 
% this is the magic script to give you the magic number
%}
% The characterized interference is then normalized in preparation for the control conditioning.
% We illiterate the normalization procedure by an example of the constant on-time buck converter.
% % The Step 1 and Step 2 follow the same normalization definitions and notations as in Section \ref{subsection:opddesignguide}.\\
% We normalize the interference frequency by the reciprocal of the off time
% \begin{align}
%     f_{n} &\triangleq \frac{1}{T_{\text{off}}} = \frac{1}{500 \times 10^{-9}\,\text{s}} = 2 \,\text{MHz},\\
%     \hat{\omega} &=  \hat{f} = \frac{f_{\text{int}}}{f_{n}} = \frac{5\,\text{MHz}}{2\,\text{MHz}} = 2.5.
% \end{align}
% We normalize the interference amplitude by the inductor current ripple
% \begin{align}
%     A_{n} &\triangleq m_1T_{\text{on}} = \frac{(V_{\text{in}} - V_{\text{out}})}{L}T_{\text{on}} \nonumber\\
%     & = \frac{(12\,\text{V} - 2\,\text{V})}{0.24\times10^{-6}\,\text{H}}\times 100\times10^{-9}\,\text{s} = 4.17 \,\text{A},\\
%     \hat{A} &= \frac{A_{\text{int}}}{A_{n}} = \frac{0.40\,\text{A}}{4.17\,\text{A}} = 0.10.
% \end{align}
% We normalize the Lipschitz constant of the interference by the inductor current ramp
% \begin{align}
%     \hat{L} = \frac{\omega_{\text{int}}A_{\text{int}}}{m_2} =  0.75.
% \end{align}
\subsection{Control Conditioning Using Slope Compensation}
% A step-by-step design guide for control conditioning is illustrated in this section. In design, we optimize the control performance given the large-signal stability constraint.

% \red{We choose a feasible ${(N_w, O_w)}$ through the tradeoff curve for settling and overshoot, and finding the optimal $\hat{m}_s$ is shown later.}
%\subsubsection{Slope Compensation} \label{subsection:sc}
% \begin{figure}
%     \centering
%     \includegraphics[width = 8 cm]{DG_sc.pdf}
%     \caption{Transient performance design diagram for the slope compensation.}
%     \label{fig:DG_sc}
% \end{figure}
\begin{comment}
The design of slope compensation include the design of 
slope $m_s$. In this constant on-time buck converter, we use the positive compensation slope to enhance the stability. For constant off-time current control loop, the compensation slope should be set as negative to enhance the stability.
We first find the range of $m_s$ to guarantee the global asymptotic stability by Corollary \ref{stabthoerem:slopecomp_constontime}.
Within this range, we next design for transient performance using the transient performance design diagram in Fig.\,\ref{fig:DG_sc}.
A practical design objective is to minimize settling time given an upper bound on the overshoot.
Depending on the interference and overshoot constraint, there might be two types of design patterns.
In pattern $A$, the overshoot constraint is loose, hence the globally minimal settling time in (\ref{eqn:th_wc_settling}) can be achieved.
In pattern $B$, the overshoot constraint is tight. The large compensation slope has to be employed, hence the settling time is sacrificed.

As shown in the case $A$ in Fig.\,\ref{fig:DG_sc}, the normalized Lipschitz constant of the interference is $0.15$ and the upper bound of overshoot is $21\,\%$. The minimal settling time occurs at the red square on the settling time --- overshoot tradeoff curve. This is also the global minimal settling time. 
In this case, the optimal compensation slope can be found from Fig.\,\ref{fig:scsettlingtime}.
We first find the settling time --- compensation slope curve given $\hat{L} = 0.15$. The optimal compensation slope $\hat{m}_s^*$ can be found at the valley of this settling time --- compensation slope curve.
As shown in the case $B$ in Fig.\,\ref{fig:DG_sc}, the normalized Lipschitz constant of the interference is $0.15$ and the constraint of overshoot is $16\,\%$.
The minimal settling time occurs at the green dot which is located at the crossing of the settling time --- overshoot trade-off curve and overshoot constraint. 
In this case, the optimal compensation slope can be found from Fig.\,\ref{fig:scovershoot}.
We first find the overshoot --- compensation slope curve given $\hat{L} = 0.15$. The optimal compensation slope $\hat{m}_s^*$ can be found at the crossing of this overshoot - compensation slope curve and the overshoot constraint.
% The practical design guide for ensuring global asymptotic stability, choosing a feasible ${(N_w, O_w)}$ through the tradeoff curve for settling and overshoot, and finding the optimal $\hat{m}_s$ is shown later in Section \ref{subsection:sc}.

We use the constant on-time buck prototype as a design example. Assume the upper bound of overshoot is $20\,\%$. To guarantee the global asymptotic stability, $\hat{m}_s$ satisfies
\begin{align}
    \hat{m}_s \ge \hat{L} -\frac{1}{2} =  0.2540.
\end{align}
From (\ref{eqn:optms}), the optimal $\hat{m}_s$ is
\begin{align}
    \hat{m}_s & = \sqrt{\frac{1}{4} + \left(2\pi \hat{\omega} \hat{A} \right)^2} - \frac{1}{2}  = 1.6936.
\end{align}
The actual compensation slope $m_s$ is
\begin{align}  \label{eqn:act_opt_slope}
    m_s = \hat{m}_s\times m_2 = 2.9582
    \,\text{A}/\mu\text{s}.
\end{align}
% In this example, given the normalized frequency and amplitude as $\omega^{*}_{\text{int}} = 1.2$ and $A^{*}_{\text{int}} = 0.3$, we have $m_s = 0.11 m_1$. 
\end{comment}
We exhibit a digital slope generator with programmable slope in Fig.\,\ref{fig:impl_sch_sc}. The slope is programmed by the increment value register $sg$. The output of the digital controller $i_{os}$ determines the offset value of the valley current. The counter $sc$ is triggered and reset every cycle. The constant-on-time modulator $sw$ resets the counter to 0 at each rising edge and freezes the counter during the entire on time.
The counter starts at the falling edge of the constant-on-time modulator $sw$ and counts upwards. $i_d$ represents the summation of the valley current offset $i_{os}$ and slope $sc$. $i_d$ is converted into an analog signal by the DAC. The output of the DAC $i_a$ is updated at the rising edge of the DAC clock. The filter smooths the stepped $i_a$ so that it is nearly an ideal ramp.
The digital slope generator and controller are implemented in the FPGA, and the DAC and filter are implemented in discrete hardware. This all-digital slope generator can be reconfigured in real-time to optimize for transient and stability at different operating points, in which gain scheduling is an example. All the critical waveforms can be found in Fig.\,\ref{fig:impl_sch_waveform}.

\begin{figure}[ht]
    \centering
    \includegraphics[width = 6cm]{impl_sch_sc.pdf}
    \caption{Schematic of the programmable digital slope generator, which allows for re-programmability and adaptability.}
    \label{fig:impl_sch_sc}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width = 8cm]{impl_sch_waveform.pdf}
    \caption{Waveform of the programmable digital slope generator shows straightforward implementation of digital functions.}
    \label{fig:impl_sch_waveform}
\end{figure}
%The digital slope generator is verified in hardware.

The output of the slope generator can function correctly both in steady state and in transition as shown in Figs.\,\ref{fig:sc_steady_10} and \ref{fig:sc_trans_10}. The slope generator output is shown in Channel 1 (dark blue). The inductor current is shown in  channel 3 (pink)  and the switching signal is shown in channel 2 (light blue). There is a propagation delay from the switching signal to the inductor current. We observe that the slope generator output is highly contaminated by the switch-on transient, but the slope compensation still functions correctly because we only need to compensate the current sensor slope during the off time, which means the switch-off transition does not induce heavy interference on the slope generator output.
\begin{figure}[ht]
\centering
    \subfigure[Steady state.]
    {
    \centering
    \includegraphics[width = 7cm]{sc_steady_10.pdf}
    \label{fig:sc_steady_10}
    }
    \subfigure[Transient.]
    {
    \centering
    \includegraphics[width = 7cm]{sc_trans_10.pdf}
    \label{fig:sc_trans_10}
    }
    \caption{Experimental waveforms of digital slope generator with slope \mbox{= 10\,A/$\mu$s} shows stable power converter operation despite a current controller corrupted by interference.}
\end{figure}

Without slope compensation, the inductor current is not stable because of the contaminated current sense voltage as illustrated in Fig.\,\ref{fig:nonsc_zoomin}.
The subharmonic frequencies of one\nobreakdash-fifth to fourth-fifths of the fundamental frequency appear in Fig.\,\ref{fig:nosc_fft}.
With slope compensation of 10\,A$/\mu$s, the inductor current is stabilized despite the severe contamination on the current sensor voltage as shown in Fig.\,\ref{fig:sc_zoomin}.
The only remaining harmonics are positive integer multiples of the fundamental frequency as validated by the Fourier spectrum in Fig.\,\ref{fig:sc_fft}.
%The steady-state inductor currents with and without the slope compensation are compared in Figs.\,\ref{fig:nonsc_zoomin} and \ref{fig:sc_zoomin}.
%The Fourier transform of the inductor current waveforms in Figs.\,\ref{fig:nosc_fft} and \ref{fig:sc_fft} are shown in Figs.\,\ref{fig:nonsc_zoomin} and \ref{fig:sc_zoomin}, respectively.
%The steady-state frequency in Figs.\,\ref{fig:nosc_fft} and \ref{fig:sc_fft} are slightly different because of the slight difference in output voltage. The hardware result verifies the theory that the inductor current can be stablized by a compensation slope.
% Note that Figure.\,\ref{fig:nonsc_zoomin} and Fig.\,\ref{fig:nosc_fft} are the same as Fig.\,\ref{fig:filterss_4_7p_zoomin} and Fig.\,\ref{fig:filterss_4_7p_zoomout} because they both are control group. 
%From the scope plot, it is not easy to capture the dynamic response of the current control loop. We export the CSV file and plot in using Matlab for better illustration. 
%The current control loop is unstable in hardware when the compensation slope is 0\,A/$\mu$s in Fig. xxx. When the slope is increased to 10\,A/$\mu$s, 
%which is closed to the design value in (\ref{eqn:act_opt_slope}). 
%the current controller settles quickly to a stable equilibrium within several cycles in Fig. xxx.
%The ringing disappears when the slope is further increased to \,A/$\mu$s. However, the current transient takes longer to settle. The transient response of the hardware agrees with theory in that there is an optimal compensation slope to optimize settling and overshoot.

The slope compensation results in a first-order response to the current control loop as illustrated in Fig.\,\ref{fig:slopetransexp}.
The greater the compensation slope, the slower the transient response as shown in Fig.\,\ref{fig:slopetranssimu}. 
%The current controller goes unstable with zero slope compensation. The current controller shows slow transient response if it is over-compensated by a slope compensation of 20\,A/$\mu$s.

% inductor current waveform
\begin{figure}[ht]
\centering
    \subfigure[Slope compensation = 0\,A/$\mu$s.]{
    \centering
    \includegraphics[width = 7cm]{nonsc_zoomin.pdf}
    \label{fig:nonsc_zoomin}
    }
    \subfigure[Slope compensation = 10\,A/$\mu$s.]{\centering
    \includegraphics[width = 7cm]{sc_zoomin.pdf}
    \label{fig:sc_zoomin}
    }
    \caption{Inductor current and current-sense voltage of a current controller corrupted by interference shows instability without slope compensation and stability.}
\end{figure}
% FFT of the inductor
\begin{figure}[ht]
\centering
    \subfigure[Slope compensation = 0\,A/$\mu$s.]
    {
    \centering
    \includegraphics[width=7 cm]{nosc_fft.pdf}
    \label{fig:nosc_fft}
    }
    \subfigure[Slope compensation = 10 A/$\mu$s.]
    {
    \centering
    \includegraphics[width=7cm]{sc_fft.pdf}
    \label{fig:sc_fft}
    }
    \caption{Fourier transform of the inductor current of the current controllers that corrupted by interference show subharmonics without slope compensation, but stable harmonics with appropriate compensation slope.}
\end{figure}
% Transient waveform
% \begin{figure}[ht]
%     \centering
%     \includegraphics[width = 6cm]{slopetransexp.pdf}
%     \caption{Experimental step-up response of the current controller with different slope compensations shows instability with no slope compensation, stability with appropriate compensation, and slow transient response with over-compensation. }
%     \label{fig:slopetransexp}
% \end{figure}
% \begin{figure}[ht]
%     \centering
%     \includegraphics[width =6cm]{slopetranssimu.pdf}
%     \caption{Hardware step-up response of the current controller with different slope compensations. The current controller goes unstable with zero slope compensation. The current controller is stabilized by a compensation slope of 5\,A/$\mu$s. The current controller shows slow transient response if it is over-compensated by a slope compensation of 20\,A/$\mu$s.}
%     \label{fig:slopetranssimu}
% \end{figure}

\begin{figure}[ht]
\centering
    \subfigure[Experimental waveforms from oscilloscope.]{
    \centering
    \includegraphics[width = 6cm]{slopetransexp.pdf}
    \label{fig:slopetransexp}
    }
    \subfigure[Experimental waveforms with the inductor current valleys marked as discrete time samples.]{\centering
    \includegraphics[width = 6cm]{slopetranssimu.pdf}
    \label{fig:slopetranssimu}
    }
    \caption{Experimental step-up response of the current control loop with different slope compensations shows instability with no slope compensation, stability with appropriate compensation, and slow transient response with over-compensation. \red{insert a picture for 10 A/mus}}
\end{figure}

\begin{comment}
\subsubsection{Low-Pass Filter}
\label{subsection:lpf}
\begin{figure}
    \centering
    \includegraphics[width = 8cm]{DG_filter.pdf}
    \caption{Transient performance design diagram for the low-pass filter.({\color{red} conservative is spelled  wrong})}
    \label{fig:no_tradeoff_lpf}
\end{figure}
We use the fist-order low-pass filter for illustration.
The design of  low-pass filter includes the design of time constant $\tau$.
We first find the range of $\tau$ to guarantee the global asymptotic stability by Theorem \ref{theorem:taomin4stability}.
Within this range, we next design for transient performance using the transient performance design diagram in Fig.\,\ref{fig:no_tradeoff_lpf}.
A practical design objective is to minimize settling time given an upper bound on the overshoot.
Depending on the interference and overshoot constraint, there might be two types of design patterns.
In pattern $A$, the overshoot constraint is loose, hence the minimal settling time can be achieved by varying the filter time constant.
In pattern $B$, the overshoot constraint is tight, hence the settling time is sacrificed.
    
As shown in the case $A$ in Fig.\,\ref{fig:no_tradeoff_lpf}, the normalized amplitude of the interference is $0.03$ and the upper bound of overshoot is $20\,\%$. The minimal settling time occurs at the green square on the performance tradeoff curve. This is also the global minimal settling time.
We first target at the settling time --- filter time constant curve which corresponds to $\hat{A} = 0.03$. The optimal filter time constant $\hat{\tau}^*$ can be found at the valley of this curve.
As shown in the case $B$ in Fig.\,\ref{fig:DG_sc}, the normalized amplitude of the interference $\hat{A} = 0.03$ and the constraint of overshoot is $16\,\%$.
In this case, the design constraints cannot be satisfied by only using comparator overdrive.
% The minimal settling time occurs at the green dot which is located at the crossing of the performance trade-off curve and overshoot constraint.

% Here we interpret (\ref{eqn:timescaleassumption2}) as
% \begin{align} \label{eqn:timescaleassumption3}
%     \omega^*_{\text{int}}\;c \ge 3.
% \end{align}
We use the constant on-time buck prototype as a design example.
We can find the range of $\tau^*$ by Theorem \ref{theorem:taomin4stability}
\begin{align}
    k_0 + A^* \; k_1 < \frac{1}{2}.
\end{align}
In this example, given $A^{*} = 0.1478$, the range of $\tau^*$ is $\tau^* \ge 0.3225 $.

We set the objective to minimize the settling with small enough overshoot. From Fig.\,\ref{fig:filter_settlingtime} and Fig.\,\ref{fig:filter_overshoot}, we choose $\tau^* = 0.5$.
% We finally verify that the selected $\tau^*$ satisfies the assumption (\ref{eqn:uplimitonc}) and (\ref{eqn:timescaleassumption}).
% The assumption (\ref{eqn:timescaleassumption}) can be equivalently expressed as
% \begin{align} \label{eqn:timescaleassumption2}
%     \omega^*\;\tau^* \ge 1.
% \end{align}
% We next verify if the product of $\omega^*$ and $\tau^*$ satisfies (\ref{eqn:timescaleassumption2}). 
In this example, given $\omega^{*} = 2.3$, $\omega^*\tau^* = 1.61 \ge 1$ satisfies the condition.
Therefore, the time constant of the low-pass filter is designed as $\tau = 0.5\,T_{\text{on}}$.

Figures \ref{fig:filterss_4_7p_zoomin}, \ref{fig:filterss_22p_zoomin} and \ref{fig:filterss_47p_zoomin} show the experimental waveforms of the current-mode buck converter with different conditioning filters. We vary the capacitor to change the time constant of first-order low-pass filter. The inductor current is shown in Channel 3 (pink) and the current sensor output is shown in Channel 1 (dark blue), which is greatly contaminated by interference. Note that the filter capacitor $C$= 4.7\,pF is always placed at the comparator input, not only for low-pass filter but also for slope compensation and comparator overdrive because it can absorb the voltage spike during the switching transitions, in the other word, limit the band-width of current-sense output. This design not only protect the comparator from saturation but also make the assumption of bandwidth limitation hold in Definition\,\ref{def:inteference}.

If only the bandwidth limiting filter is used, the converter cannot function properly because inductor current exhibits a complicated subharmonic behavior as shown in Fig.\, \ref{fig:filterss_4_7p_zoomin}. From the Fourier transform of inductor current in Fig.\,\ref{fig:filterss_4_7p_zoomout}, we 
observe that besides the switching frequency component, the $1/5^{\text{th}}$, $2/5^{\text{th}}$, $3/5^{\text{th}}$, $4/5^{\text{th}}$ order subharmonics are also commingled because of the interference.
We increase the time constant of low-pass filter by increasing the capacitance to 22\,pF. As shown in Fig.\,\ref{fig:filterss_22p_zoomin}, the inductor current goes back to stable periodic steady state. Figure\,\ref{fig:filterss_22p_zoomout}, a longer-horizon view, further confirms our observation. The Fourier transform of inductor current only contains switching-frequency and higher-order harmonics. A further step to increase the capacitance to 68\,pF destabilizes the inductor current as shown in Fig.\,\ref{fig:filterss_47p_zoomin}. Figure\,\ref{fig:filterss_47p_zoomout} shows that different from  Fig.\,\ref{fig:filterss_4_7p_zoomin}, the unstable inductor current in Fig.\,\ref{fig:filterss_47p_zoomin} only contains the $1/2^{\text{th}}$ order subharmonics. The experimental steady state of current controller matches the theory. A fast filter cannot attenuate the interference and decrease the nonlinearity of current mapping. A slow filter can distort the linear ramp and increase the nonlinearity of current mapping.

The low-pass filter affects the transition of current controller. We test the step-up response of the current controller under four different conditioning filters as shown in Fig.\,\ref{fig:filtertransexp}.  For better illustration, we export the oscilloscope data to Matlab and plot them in Fig.\,\ref{fig:filtertranssimu}. The valley current are annotated because we are directly controlling valley current in buck converter using constant-on time control. When $C_f = 4.7$\,pF results in an unstable steady state. The current controller is stabilized when the filter capacitor is increased to $C_f = 22$\,pF. However, it takes around 10 cycles for current controller to fully settle down. The settling transition is faster when the filter capacitor is elevated to $C_f = 47$\,pF. However, there exists a relatively big overshoot during transition, which can be explained by the extra zero introduced by filter. When $C_f = 68$\,pF, the current controller finally loses stability and evolves into a 2-cycle periodic steady state. The experimental transition of current controller matches the theory that there exist optimal filter time constant to optimize the settling and overshoot.

\begin{figure}[ht]
    \subfigure[$C$= 4.7\,pF,\,$R$ =  730\,$\Omega$]{
    \centering
    \includegraphics[width = 8 cm]{filterss_4_7u_zoomin.PNG}
    \label{fig:filterss_4_7p_zoomin}
    }
    \newline
    \subfigure[$C$= 22\,pF,\,$R$ =  730\,$\Omega$]{
    \centering
    \includegraphics[width = 8 cm]{filterss_22u_zoomin.png}
    \label{fig:filterss_22p_zoomin}
    }
    \newline
    \subfigure[$C$= 68\,pF,\,$R$ =  730\,$\Omega$]{
    \centering
    \includegraphics[width = 8 cm]{filterss_68u_zoomin.PNG}
    \label{fig:filterss_47p_zoomin}
    }
    \caption{Inductor current and current-sense output of the current controllers with different filters.}
\end{figure}
\begin{figure}[ht]
    \subfigure[$C$= 4.7\,pF,\,$R$ =  730\,$\Omega$]{
    \centering
    \includegraphics[width = 8 cm]{filterss_4_7u_zoomout.pdf}
    \label{fig:filterss_4_7p_zoomout}
    }
    \newline
    \subfigure[$C$= 22\,pF,\,$R$ =  730\,$\Omega$]{
    \centering
    \includegraphics[width = 8 cm]{filterss_22u_zoomout.pdf}
    \label{fig:filterss_22p_zoomout}
    }
    \newline
    \subfigure[$C$= 68\,pF,\,$R$ =  730\,$\Omega$]{
    \centering
    \includegraphics[width = 8 cm]{filterss_68u_zoomout.pdf}
    \label{fig:filterss_47p_zoomout}
    }
    \caption{Fourier transform of the inductor current of the current controllers with different filters.}
\end{figure}
\begin{figure}[ht]
    \centering
    \includegraphics[width = 8 cm]{filtertransexp.pdf}
    \caption{Experimental step-up response of the current controller with different filters.}
    \label{fig:filtertransexp}
\end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[width = 8 cm]{filtertranssimu.png}
    \caption{Step-up response of the current controller with different filters.}
    \label{fig:filtertranssimu}
\end{figure}
\end{comment}
% step 3.3
\begin{comment}
\subsubsection{Comparator-Overdrive-Delay Conditioning} \label{subsection:opddesignguide}
There are several ways to approach designing comparator-overdrive-delay conditioning.  The most straightforward method is to use a nomogram to determine the comparator time constant $\tau$ from interference parameters $\hat{A}$ and $\hat{\omega}$.  
The second method is to directly use Theorems\,\ref{theorem:gmax4stability} and \ref{theorem:gmax4overdrivedelay} in Section\,\ref{section:opd}.

The nomogram, as shown in Figs.\,\ref{fig:copd_nomogram_p1}, \ref{fig:copd_nomogram_p2} and \ref{fig:copd_nomogram_p3}, allows you to design a stable control loop for the constant on/off-time current-mode converter.
% we provide an alternative nomogram method so that a designer can select the comparator time constant more conveniently.
The $x$-axis of nomogram takes use of the lower bound on frequency $\omega_l$ of interference.
The $y$-axis of nomogram takes use of the upper bound on amplitude $A_{ub}$ of interference.
All values in the nomogram are normalized.
Figures \ref{fig:copd_nomogram_p1} and \ref{fig:copd_nomogram_p2} share the same $x$\,-\,axis but has different $y$\,-\,axis ranges because the trend of the contour changes when the interference frequency increases.
Figure\;\ref{fig:copd_nomogram_p1} describes the case when the interference frequency is below the switching frequency.\footnote{For the constant on(off)-time operation, this means the reciprocal of on(off) time, i.e. the fastest switching frequency.}
As the amplitude of interference increases, the required comparator time constant increases.
As the frequency of interference decreases, the required comparator time constant increases.
Figure\;\ref{fig:copd_nomogram_p2} describes the case when the interference frequency is higher than the switching frequency. 
The asymptotic contour line is almost vertical.
This means that the interference amplitude mainly determines the required comparator time constant.
Both Fig.\;\ref{fig:copd_nomogram_p1} and Fig.\;\ref{fig:copd_nomogram_p2} show that as the amplitude of interference increases, the required comparator time constant increases. 
The intuition behind it is when as the interference becomes more severe, we need a  ``slower'' and ``softer'' comparator to condition the interference.

Using the constant on-time buck hardware prototype as a design example, we can observe in Fig.\,\ref{fig:copd_nomogram_p2} that the interference parameters that appear in the nomogram result in the normalized comparator time constant $\hat{\tau} \ge 0.12$.

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width = 8 cm]{design_comp.pdf}
%     \caption{Design Example for Comparator Overdrive.}
%     \label{fig:comp_design_example}
% \end{figure}

The product of the trigger voltage and comparator time constant should be
\begin{align}
     V_{\text{trig}}\tau = R_{\text{sample}}\frac{1}{2}m_2 T_{\text{off}}^2\,\hat{\tau} \ge 1061 \,\text{mV}\cdot\text{ns}.
\end{align}

The results of the design in Fig.\,\ref{fig:copd_nomogram_p2} for the buck converter prototype can be observed in Fig.\,\ref{fig:c_comp}. 
%To illustrate the how hardware demonstration of the %comparator,
The current control loop using the comparator LT1711 \cite{Dual2001}, whose time constant --- trigger voltage product is lower than the minimum value, behaves unstable.
The current control loop using the comparator AD8469 \cite{Devices}, whose time constant --- trigger voltage product is lower than the minimum value, behaves stable. The datasheet does not explicitly provide the time constant $\tau$, instead, it includes the overdrive delay diagram as shown in Figs.\,\ref{fig:simumodelcomp_lt1711} and \ref{fig:simumodelcomp_ad8469}. We fitted the data sheet by the linear regression equation.
\begin{align}
    t_{od} = p_1 \frac{1}{V_{od}} + p_2.
\end{align}
$p_1$ is the fitted time constant - trigger voltage product and $p_2$ is the fitted constant propagation delay.

% We choose two types of comparator with different overdrive delay --- LT1711 \cite{Dual2001} and AD8469 \cite{Devices}. 
% LT1711 is an ultra-fast comparator with the overdrive delay ranging from 4\,ns to 6\,ns. The time constant --- trigger voltage product of AD8469 is 6.1\,ns$\cdot$mV which is smaller than the upper bound. AD8469 has the overdrive delay ranging from  25\,ns to 50\,ns. The time constant --- trigger voltage product of AD8469 is 113.17\,ns$\cdot$mV which is bigger than the upper bound. Both comparator have short enough propagation delay so that the closed-loop dynamics is not affected.

Using Theorems\,\ref{theorem:gmax4stability} and \ref{theorem:gmax4overdrivedelay}, the designer can design the constant off-time current-mode converter for additional objectives including the small-signal and large-signal transient performance.
The design equations of constant on-time current-mode converter, fixed-frequency peak current-mode converter, fixed-frequency valley current-mode converter are provided in the appendix respectively. 
The choice of regions from I to IV and the design of comparator time constant $\tau$.
If we are not sure about choosing the region from I to IV, we can always shift the boundaries of regions to the right to get the conservative design. The price we paid is the longer delay time. 

We first find the range of $\tau$ to guarantee the global asymptotic stability by Theorem \ref{theorem:gmax4stability}. Within this range, we next design for transient performance using the transient performance design diagram in Fig.\,\ref{fig:opdr_settling_overshoot}.
A practical design objective is to minimize the minimum on~time $T_{\text{\text{on}}}^{\text{min}}$ given an upper bound on the overshoot and $T_{\text{\text{on}}}^{\text{min}}$.
Depending these constraints, there exist two types of design patterns.
In pattern $A$, there exist feasible comparator time constants given the constraints. We then pick up the comparator time constant which minimizes the $T_{\text{\text{on}}}^{\text{min}}$.
% The minimum $T_{\text{\text{on}}}^{\text{min}}$ is always achieved when the comparator time constant is at the lower bound. This observation matches our intuition because if the overdrive delay is longer, the interference attenuation ability of comparator is better, hence the overshoot and settling time is smaller.
In pattern $B$, the constraints on the overshoot and $T_{\text{\text{on}}}^{\text{min}}$ do not result in any feasible comparator time constant.

% {\color{blue} think about where to put this sentences: in the design guide, don't put the set point so it is at the actuator operating point bound}
As shown in the case $A$ in Fig.\,\ref{fig:no_tradeoff_copd_oo}, the normalized amplitude of the interference is $0.02$, the upper bound of overshoot is $40\,\%$ and the upper bound of the normalized $T_{\text{\text{on}}}^{\text{min}}$ is $0.6$.
% The minimum settling time occurs at the green square on the settling time --- comparator overdrive delay tradeoff curve.
In this case, the optimal comparator time constant can be found by the following procedures:
\begin{enumerate}
\item Find the optimal $\hat{T}_{\text{\text{on}}}^{\text{min}} = 0.42$ in overshoot --- overdrive delay curve in Fig.\,\ref{fig:no_tradeoff_copd_oo}.
\item Given $\hat{A} = 0.02$, locate the comparator time constant --- overdrive delay curve in Fig.~\ref{fig:opdr_overdrive_delay}.
\item Find the optimal comparator time constant $\hat{\tau}^*$ in the curve.
\end{enumerate}

As shown in the case $B$ in Fig.\,\ref{fig:no_tradeoff_copd_oo}, the normalized interference amplitude is $0.03$, the upper bound of overshoot is $5\,\%$ and the upper bound of $\hat{T}_{\text{\text{on}}}^{\text{min}}$ is $1$. 
In this case, the design constraints cannot be satisfied by only using comparator overdrive.
% The design of comparator overdrive includes the design of comparator time constant $\tau$.
%% the nomogram 
\begin{figure*}[t]
\centering
\subfigure[Interference frequency \text{$\hat{\omega} \in [0.1,1]$}
\newline (increase the fonts)]{\includegraphics[width=0.3\textwidth]{section3/opd/nomogram_p1_c.pdf} 
\label{fig:copd_nomogram_p1}
%\caption{Interference frequency }
}
\subfigure[Interference frequency \text{$\hat{\omega} \in [1,3]$}
\newline (increase the fonts)]{
    \includegraphics[width=0.3\textwidth]{    design_comp.pdf}
    %\rule{4cm}{3cm}
   \label{fig:copd_nomogram_p2}
   %\caption{Interference frequency $\omega_{\text{int}} \in [0.5,3]$}
}
\subfigure[Interference frequency \text{$\hat{\omega} \in [0.1,3]$}
\newline (increase the fonts)]{
    \includegraphics[width=0.3\textwidth]{section3/opd/nomogram_p3_c.pdf}
    %\rule{4cm}{3cm}
   \label{fig:copd_nomogram_p3}
   %\caption{Interference frequency $\omega_{\text{int}} \in [0.5,3]$}
}
\caption{The design nomogram for comparator overdrive.}
\end{figure*}
% The practical design guide for ensuring global asymptotic stability, choosing a feasible ${(N_w, O_w)}$ through the tradeoff curve for settling and overshoot, and finding the optimal $\hat{m}_s$ is shown later in Section \ref{subsection:sc}.
% \begin{figure}
%     \centering
%     \includegraphics[width = 8 cm]{no_tradeoff_copd_so.pdf}
%     \caption{Transient performance design diagram I for comparator overdrive.}
%     \label{fig:no_tradeoff_copd_so}
% \end{figure}
\begin{figure}
    \centering
    \includegraphics[width = 8 cm]{no_tradeoff_copd_oo.pdf}
    \caption{Transient performance design diagram for comparator overdrive.{\color{red}overdrive delay should be normalized.}}
    \label{fig:no_tradeoff_copd_oo}
\end{figure}
% We would like to introduce a step-by-step design guide for the overdrive propagation delay technique.
% \noindent Step 1: We normalize the interference frequency by the reciprocal of the on-time
% \begin{align}
%     \omega_{n} &\triangleq \frac{2 \pi}{T_{\text{on}}} = \frac{2 \pi}{383 \times 10^{-9}\,\text{s}} =1.64\times 10^{7}\,\text{s}^{-1},\\
%      \omega^{*} &= \frac{\omega_{\text{int}}}{\omega_{n}} = \frac{3.77\times 10^{7}\,\text{s}^{-1}}{1.64 \times 10^{7}\,\text{s}^{-1}} = 2.30.
% \end{align}
% Step 2: We normalize the interference 
% amplitude by the inductor current ripple
% \begin{align}
%     A_{n} &\triangleq m_1T_{\text{on}} = \frac{(V_{\text{out}} - V_{\text{in}})}{L}T_{\text{off}} \nonumber\\
%     & = \frac{(35\,\text{V} - 12\,\text{V})}{6.80\times10^{-6}\,\text{H}}\times200\times10^{-9}\,\text{s} = 6.77 \times 10^{-1}\,\text{A},\\
%     A^* &= \frac{A_{\text{int}}}{A_{n}} = \frac{0.10\,\text{A}}{6.77 \times 10^{-1}\,\text{A}} = 1.48 \times 10^{-1}.
% \end{align}
% The minimum normalized time constant $\tau$ can be obtained from the Figure as
% \begin{align}
%   k_n \triangleq \frac{m_1}{\omega_n^2 V_{\text{th}}}K_1 \left(\frac{A_n\omega_n}{m_1}\right) & = \frac{1.77 \times 10^6}{(1.64\times 10^{7})^2 \times 1}K_1 \left(2\pi\right)\nonumber \\
%   & = 1.64\times10^{-7}.
% \end{align}

% we can uniquely determine the purple point on the nomogram and read the lower bound on comparator time constant.
% \begin{figure}
%     \centering
%     \includegraphics[width=8 cm]{Drawnomogram_reachability_0_5_3_example.pdf}
%     \caption{Comparator overdrive design example.}
%     \label{fig:mynomogram_p3}
% \end{figure}
% As shown in Fig.\;\ref{fig:mynomogram_p3}, we denote the distance between the purple point to the left adjacent contour $d_1$ and the distance between the purple point to the right adjacent contour $d_2$. The ratio $d_1/d_2$ is roughly 2:\,7.
% The maximum gain $G_{\text{max}}$ can be calculated as
% \begin{align}
%     G_{\text{max}} = \frac{1}{k^* \times k_n} = \frac{1}{0.02778 \times 1.644\times10^{-7}} = 2.190\times10^8.
% \end{align}

% Figure.\,\ref{fig:c_comp} shows that the current controller with LT1711 goes unstable. By changing the comparator to AD8469, the inductor current only contains the switching frequency component, indicating a stable current controller. Note that in selection of comparator, it is not the minimum propagation delay but the dynamic range of overdrive that determines the stablization effect of comparator.


\begin{figure}[ht]
    \subfigure[LT1711]
    {\centering
    \includegraphics[width = 8cm]{complt1711.pdf}
    \label{fig:complt1711}
    }
    \newline
    \subfigure[AD8469]
    {\centering
    \includegraphics[width = 8 cm]{comp_da_8469.pdf}
    \label{fig:comp_da_8469}
    }
    \caption{Fourier transform of the inductor current of the current controllers with different comparators. The current controller goes unstable when the comparator with shorter overdrive delay (LT1711) is used. The current controller is stable when the comparator with longer overdrive delay (AD8469) is used.}
    \label{fig:c_comp}
\end{figure}
\end{comment}

% \subsection{Future Extensions}
% The theory developed in this paper can be extended towards but not limited to the following directions:
% 1)\,the converter using the fixed-frequency peak current control or constant off-time control can operate in Discontinuous Conduction Mode (DCM) if the load current is low.
% It is not hard to prove that if we design a stable current control loop in Continuous Conduction Mode (CCM), it is guaranteed to be stable in DCM.
